Multimodal Large Language Models for Text-rich Image Understanding: A Comprehensive Review

The recent emergence of Multi-modal Large Language Models (MLLMs) has introduced a new dimension to the Text-rich Image Understanding (TIU) field, with models demonstrating impressive and inspiring performance. However, their rapid evolution and widespread adoption have made it increasingly challenging to keep up with the latest advancements. To address this, we present a systematic and comprehensive survey to facilitate further research on TIU MLLMs. Initially, we outline the timeline, architecture, and pipeline of nearly all TIU MLLMs. Then, we review the performance of selected models on mainstream benchmarks. Finally, we explore promising directions, challenges, and limitations within the field.

==> MLLM_OCR/Table/MLLM.tex <==
    \centering
    \scriptsize
    \begin{tabular}{l|>{\centering\arraybackslash}m{3.cm}>{\centering\arraybackslash}m{2.cm}>{\centering\arraybackslash}m{1.7cm}|>{\centering\arraybackslash}m{1.6cm}|>{\centering\arraybackslash}m{0.6cm}>{\centering\arraybackslash}m{0.6cm}>{\centering\arraybackslash}m{0.6cm}>{\centering\arraybackslash}m{0.8cm}|>{\centering\arraybackslash}m{0.6cm}}
    \toprule
    Model & Visual Encoder & Modality Connector & LLM Decoder & Training Pipline & DocVQA & InfoVQA & ChartQA & TextVQA & Avg. \\
   \midrule
    % Flamingo (2022) & NFNet-F6 & Cross-attention & Chinchilla-1.4B/7B/70B & - & - & -\\
   % \midrule 
    % BLIP-2 (2023) & CLIP/Eva-CLIP ViT@224 & Q-Former w/ MLP & Flan-T5/OPT & - & - & -\\
   % \midrule 
   UReader~\cite{ye2023ureader} & CLIP-ViT-L/14 & Cross Attention & LLaMA-7B & MA+IA & 65.4 & 42.2 & 59.3 & 57.6 &56.13 \\
   DocLLM-1B~\cite{Wang2023ARXIV_DocLLM_A_layout} & - & - & Falcon-1B & MA+IA & 61.4 & - & - & - & -\\
    DocLLM-7B~\cite{Wang2023ARXIV_DocLLM_A_layout} & - & - & LLaMA2-7B & MA+IA & 69.5 & - & - & - &-\\

    Cream \cite{kim2023visually}& CLIP-ViT-L/14 & Cross Attention & Vicuna-7B & MA+IA & 79.5 & 43.5 & 63.0 & - &- \\
    % \color{red}{ICL-D3IE} \cite{he2023icl} & - & - & ChatGPT & IA & - & - & - & - \\
   % InternVL1.2-40B & InternViT-6B & MLP & Nous-Hermes-2-Yi-34B & MA+IA & 57.7 & 39.5 & 68.0 & 72.5 \\
    
    % LLaVA-7B~\cite{liu2023llava} & CLIP-ViT-L/14 & MLP & Vicuna-7B & MA+IA & - & - & - & - \\
    LLaVA-13B~\cite{liu2023llava} & CLIP-ViT-L/14 & MLP & Vicuna-13B & MA+IA & 6.9 & - & - & 36.7 & -\\
   % \midrule 
    % MiniGPT-4~\cite{zhu2023minigpt} & Eva-CLIP ViT-G/14 & Q-Former w/ MLP & Vicuna-13B & MA+IA & - & - & - & -\\
   % \midrule 
    % mPLUG-Owl~\cite{ye2023mplug_owl}& CLIP ViT-L/14 & Cross-attention & LLaMA-7B & MA+IA & - & - & - & -\\
   % \midrule 
    % Otter (2023) & CLIP ViT-L/14 & Cross-attention & LLaMA-7B & - & - & -\\
   % \midrule 
    % X-LLM (2023) & ViT-G; A: C-Former & Q-Former w/ MLP & ChatGLM-6B & - & - & -\\
   % \midrule 
    % VideoChat (2023) & ViT-G & Q-Former w/ MLP & Vicuna & - & - & -\\
   % \midrule 
    % InstructBLIP (2023) & ViT-G/14@224 & Q-Former w/ MLP & Flan-T5/Vicuna & - & - & -\\
   % \midrule 
    % PandaGPT (2023) & ImageBind & MLP & Vicuna-13B & - & - & -\\
   % \midrule 
    % GILL (2023) & CLIP ViT-L & MLP & OPT-6.7B & - & - & -\\
   % \midrule 
    PaLI-X~\cite{chen2023pali} & ViT-22B & MLP & UL2-32B & MA+IA & 86.8 & 54.8 & 72.3 & 80.8  & 73.68\\
   % \midrule 
    % Video-LLaMA (2023) & Eva-CLIP ViT-G/14; A: ImageBind & Q-Former w/ MLP & Vicuna/LLaMA & - & - & -\\
   % \midrule 
    % Video-ChatGPT (2023) & CLIP ViT-L/14 & MLP & Vicuna-v1.1 & - & - & -\\
   % \midrule 
    % Shikra (2023) & CLIP ViT-L/14@224 & MLP & Vicuna-7B/13B & - & - & -\\
   % \midrule 
    LLaVAR~\cite{zhang2023llavar}& CLIP-ViT-L/14 & MLP & Vicuna-13B & MA+IA & 11.6 & - & - & 48.5 & -\\
   % \midrule 
    % mPLUG-DocOwl (2023) & CLIP ViT-L/14 & Cross-attention & LLaMA-7B & - & - & -\\
   % \midrule 
    % Lynx (2023) & Eva-CLIP ViT-1B & Cross-attention & Vicuna & - & - & -\\
   % \midrule 
    % Emu (2024) & Eva-CLIP-1B & Cross-attention & LLaMA-13B & - & - & -\\
   % \midrule 
    % DLP (2023) & CLIP/Eva-CLIP ViT & Q-\&P-Former w/ MLP & OPT/Flan-T5 & - & - & -\\
   % \midrule 
    % BuboGPT (2023) & CLIP/Eva-CLIP ViT; A: ImageBind & Q-Former w/ MLP & Vicuna & - & - & -\\
   % \midrule 
    % ChatSpot (2023) & CLIP ViT-L/14 & MLP & Vicuna-7B/LLaMA & - & - & -\\
   % \midrule 
    
   % \midrule 
    Qwen-VL~\cite{bai2023qwenvl} & ViT-bigG & Cross Attention & Qwen-7B & MA+IA & 65.1 & 35.4 & 65.7 & 63.8 &57.50\\
   % \midrule 
    % LaVIT (2024) & ViT & Cross-attention & LLaMA-7B & - & - & -\\
   % \midrule 
    % NExT-GPT (2023) & I/V/A: ImageBind & MLP & Vicuna-7B & - & - & -\\
   % \midrule 
    % DreamLLM (2024) & CLIP ViT-L & MLP & Vicuna & - & - & -\\
   % \midrule 
    % AnyMAL (2023) & CLIP ViT/L\&ViT-G\&DinoV2; V: Intervideo; A: CLAP & Cross-attention; A: MLP & LLaMA-2 & - & - & -\\
   % \midrule 
    % MiniGPT-5 (2023) & Eva-CLIP ViT-G/14 & Q-Former w/ MLP & Vicuna-7B & - & -& - & - & -\\
   % \midrule 
    LLaVA-1.5-7B~\cite{liu2023improvedllava} & CLIP-ViT-L & MLP & Vicuna1.5-7B & MA+IA & - & - & - & 58.2 &- \\
    LLaVA-1.5-13B~\cite{liu2023improvedllava} & CLIP-ViT-L & MLP & Vicuna1.5-13B & MA+IA & - & - & - & 62.5 &- \\
    % SPHINX~\cite{lin2023sphinx} & CLIP-ViT+CLIP-ConvNext+DINOv2-ViT+Q-Former & MLP & LLaMA2-7B & MA+IA & - & - & - & 61.2 \\
    CogAgent~\cite{hong2023cogagent} & EVA2-CLIP  & MLP+Cross Attention & Vicuna-13B & MA+IA & 81.6 & 44.5 & 68.4 & 76.1 & 67.65\\
    Unidoc~\cite{feng2023unidoc} & CLIP-ViT-L/14 & MLP & Vicuna-13B & MA+IA & 90.2 & 36.8 & 70.5 & 73.7 & 67.80 \\
    
  %  LLaVA-OneVision~\cite{li2024llavaonevisioneasyvisualtask} & SigLIP & MLP & Qwen2-7B & MA+IA & 87.5 & 68.8 & 80.0 & - \\
   % \midrule 
    % MiniGPT-v2 (2023) & Eva-CLIP ViT & MLP & LLaMA-2-Chat-7B & - & - & - & - & -\\
   % \midrule 
    % CogVLM (2023) & Eva-2-CLIP ViT & MLP & Vicuna-v1.5-7B & - & - & - & - & -\\
   % \midrule 
    % Qwen-Audio (2023) & A: Whisper-L-v2 & MLP & Qwen-7B & - & - & -\\
   % \midrule 
    % DRESS (2023) &Eva-CLIP ViT-G/14 & MLP & Vicuna-v1.5-13B & - & - & -\\
   % \midrule 
    % X-InstructBLIP (2023) & Eva-CLIP ViT-G/14; A: BEATs; 3D: ULIP-2 & Q-Former w/ MLP & Vicuna-v1.1-7B/13B & - & - & -\\
   % \midrule 
    % CoDi-2 (2023) & I/V/A: ImageBind & MLP & LLaMA-2-Chat-7B & - & - & -\\
   % \midrule 
    % RLHF-V (2023) & BEiT-3 & MLP & Vicuna-v1-13B & - & - & -\\
   % \midrule 
    % Silkie (2023) & ViT initialized from OpenCLIP's ViT-bigG & Cross-attention & Qwen-7B & - & - & -\\
   % \midrule 
    % Lyrics (2023) & CLIP ViT-L/14\&Grounding-DINO-T \&SAM-HQ\&ViT-H\&RAM++ & MQ-Former w/ Linear Projection & Vicuna-13B & - & - & -\\
   % \midrule 
    % VILA (2023) & ViT@336 & MLP & LLaMA-2-7B/13B & - & - & -\\
   % \midrule 
   % InternVL~\cite{chen2024internvlscalingvisionfoundation} & InternViT-6B & Cross Attention \& MLP & QLLaMA-8B \& Vicuna-13B & MA+IA & - & - & - & -\\
   % \midrule 
    % ModaVerse (2024) & ImageBind & MLP & LLaMA-2 & - & - & -\\
   % \midrule 
    % MM-Interleaved (2024) & CLIP ViT-L/14 & Cross-attention & Vicuna-13B & - & - & -\\
   % \midrule 
    Monkey~\cite{Li2024CVPR_Monkey_Image_Resolution} & Vit-BigG & Cross Attention & Qwen-7B & MA+IA & 66.5 & 36.1 & 65.1 & 67.6 & 58.83\\
   % \midrule 
    Mini-Monkey~\cite{Huang2024ARXIV_Mini_Monkey_Alleviating} & InternViT-300M & MLP & InternLLM2-2B & IA & 87.4 & 60.1 & 76.5 & 75.7 & 74.93\\
   % \midrule 
    TextMonkey~\cite{Liu2024ARXIV_TextMonkey_An_OCR} & Vit-BigG & Cross Attention & Qwen-7B & MA+IA & 73.0 & - & 66.9 & 65.6 & -\\
    IDEFICS2 (\cite{laurençon2024mattersbuildingvisionlanguagemodels}) & SigLIP-SO400M & Cross Attention & Mistral-7B & MA+IA & 74.0 & - & - & 73.0 & -\\
   % \midrule 
    LayoutLLM~\cite{luo2024layoutllm} & LayoutLMv3-large & MLP & Vicuna1.5-7B & MA+IA & 74.25 & - & - & - & -\\
   % \midrule 
    DocKylin~\cite{zhang2024dockylin} & Swin & MLP & Qwen-7B & MA+IA & 77.3 & 46.6 & 66.8 & - & -\\
   % \midrule 
    DocLayLLM~\cite{liao2024doclayllm}  & LayoutLMV3 & MLP & LLaMA3-8B & MA+IA & 77.79 & 42.02 & - & - & -\\
   % \midrule 
    mPLUG-DocOwl ~\cite{Hu2024ARXIV_mPLUG_DocOwl_1}  & CLIP-ViT-L/14 & Cross Attention & LLaMA-7B & MA+IA & 62.2 & 38.2 & 57.4 & 52.6 & 52.60\\
   % \midrule 
    mPLUG-DocOwl1.5 ~\cite{hu2024mplug_docowl1.5_arxiv}  & CLIP-ViT-L/14  & H-Reducer & LLaMA2-7B & MA+IA & 82.2 & 50.7 & 70.2 & 68.6 & 67.93\\
   % \midrule 
    mPLUG-DocOwl2 ~\cite{Hu2024ARXIV_mPLUG_DocOwl2_High}  & CLIP-ViT-L/14  & H-Reducer & LLaMA2-7B & MA+IA & 80.7 & 46.4 & 70.0 & 66.7 & 65.95\\
   % \midrule 
    Vary~\cite{wei2024vary}  & CLIP-ViT-L/14 + SAM & MLP & Qwen-7B & MA+IA & 76.3 & - & 66.1 & - & -\\
    Eagle~\cite{shi2024eagleexploringdesignspace}  & CLIP + ConvNeX + Pix2Struct + EVA2 + SAM & MLP & LLaMA3-8B & MA+IA & 86.6 & - & 80.1 & 77.1 & -\\
    
    PDF-WuKong~\cite{Xie2024ARXIV_PDF_WuKong_A} & CLIP-ViT-L-14 & Cross Attention & InernLM2-7B & MA+IA & 85.1 & 61.3 & 80.0 & - & -\\
    InstructDoc~\cite{tanaka2024instructdoc} & CLIP/Eva-CLIP-ViT & Cross Attention + MLP & Flan-T5/OPT & MA+IA & - & 50.9 & 29.4 & 53.8 &-\\
    
    TextHawk~\cite{yu2024texthawk}  & SigLIP & Cross Attention & InternLM-XComposer & MA+IA & 76.4 & 50.6 & 66.6 & -&-\\
    TextHawk2~\cite{yu2024texthawk2}  & SigLIP & Cross Attention & Qwen2-7B & MA+IA & 89.6 & 67.8 & 81.4 & 75.1 &78.48\\
    % MM1 & ViT-H & C-Abstractor & - & - & 76.8 & - & - & - \\
    MM1.5-1B~\cite{zhang2024mm1_5} & CLIP-ViT-H & C-Abstractor & Private & MA+IA & 81.0 & 50.5 & 67.2 & 72.5 &67.80\\
    MM1.5-3B~\cite{zhang2024mm1_5} & CLIP-ViT-H & C-Abstractor & Private & MA+IA & 87.7 & 58.5 & 74.2 & 76.5 & 74.23\\
    MM1.5-7B~\cite{zhang2024mm1_5} & CLIP-ViT-H & C-Abstractor & Private & MA+IA & 88.1 & 59.5 & 78.6 & 76.5 & 75.68\\
    MM1.5-30B~\cite{zhang2024mm1_5} & CLIP-ViT-H & C-Abstractor & Private & MA+IA & 91.4 & 67.3 & 83.6 & 79.2 & 80.38\\
    HRVDA~\cite{liu2024hrvda} & Swin-L & MLP & LLaMA2-7B & MA+IA & 72.1 & 43.5 & 67.6 & 73.3 & 64.13\\
    % LayoutLLM (2024)  & LayoutLMv3 with DocPTM & MLP & Vicuna-7B-v1.5 & - & 74.3 & - & - & - \\
    InternVL1.5-26B~\cite{chen2024far} & InternViT-6B & Pixel-shuffle + MLP & InternLM2-20B & MA+IA & 90.9 & 72.5 & 83.8 & 80.6 & 81.95\\
   % InternVL2-1B & InternViT-300M & MLP & Qwen2-0.5B & MA+IA & 81.7 & 50.9 & 72.9 & 70.5 \\
  %  InternVL2-2B & InternViT-300M & MLP & InternLM2-1.8B & MA+IA & 86.9 & 58.9 & 76.2 & 73.3 \\
  %  InternVL2-4B & InternViT-300M & MLP & Phi-3-mini & MA+IA & 89.2 & 67.0 & 81.5 & 74.4 \\
  %   InternVL2-8B & InternViT-300M & MLP & InternLM2.5-7B & MA+IA & 91.6 & 74.8 & 83.3 & 77.4 \\
  %  InternVL2-26B & InternViT-6B & MLP & InternLM2-20B & MA+IA & 92.9 & 75.9 & 84.9 & 82.3 \\
  %  InternVL2-40B & InternViT-6B & MLP & Nous-Hermes-2-Yi-34B & MA+IA & 93.9 & 78.7 & 86.2 & 83.0 \\
    % InternVL2-108B & InternViT-6B & MLP & Qwen2-0.5B-Instruct & MA+IA & - & - & - & - \\
    InternVL2.5-1B~\cite{chen2024internvl2_5} & InternViT-300M & Pixel-shuffle + MLP & Qwen2.5-0.5B & MA+IA & 84.8 & 56.0 & 75.9 & 72.0 & 72.18\\
    InternVL2.5-2B~\cite{chen2024internvl2_5} & InternViT-300M & Pixel-shuffle + MLP & InternLM2.5-1.8B & MA+IA & 88.7 & 60.9 & 79.2 & 74.3 & 75.78\\
    InternVL2.5-4B~\cite{chen2024internvl2_5} & InternViT-300M & Pixel-shuffle + MLP & Qwen2.5-3B & MA+IA & 91.6 & 72.1 & 84.0 & 76.8 & 81.13 \\
    InternVL2.5-8B~\cite{chen2024internvl2_5} & InternViT-300M & Pixel-shuffle + MLP & InternLM2.5-7B & MA+IA & 93.0 & 77.6 & 84.8 & 79.1 & 83.63 \\
    InternVL2.5-26B~\cite{chen2024internvl2_5} & InternViT-6B & Pixel-shuffle + MLP & InternLM2.5-20B & MA+IA & 94.0 & 79.8 & 87.2 & 82.4 & 85.85 \\
    InternVL2.5-38B~\cite{chen2024internvl2_5} & InternViT-6B & Pixel-shuffle + MLP & Qwen2.5-32B & MA+IA & 95.3 & 83.6 & 88.2 & 82.7 & 87.45\\
    InternVL2.5-78B~\cite{chen2024internvl2_5} & InternViT-6B & Pixel-shuffle + MLP & Qwen2.5-72B & MA+IA & 95.1 & 84.1 & \cellcolor{gray!30}\textbf{88.3} & 83.4 & 87.73 \\
    InternVL2.5-8B-mpo\cite{wang2024enhancingreasoningabilitymultimodal}$\dagger$  & InternViT-300M & Pixel-shuffle +MLP & InternLM2.5-7B & PA & 92.3 & 76.0 & 83.8 & 79.1 & 82.80 \\
    DocPeida~\cite{Feng2024ARXIV_DocPedia_Unleashing_the} & Swin & MLP & Vicuna-7B & MA+IA & 47.1 & 15.2 & 46.9 & 60.2 & 42.35 \\
    TinyChart~\cite{zhang2024tinychart} & SigLIP & MLP & Phi-2 & IA & - & - & 83.6 & - & - \\
    TokenPacker-7B~\cite{li2024tokenpackerefficientvisualprojector} & CLIP-ViT-L/14 & Cross Attention & Vicuna-7B & MA+IA & 60.2 & - & - & - & - \\
    TokenPacker-13B~\cite{li2024tokenpackerefficientvisualprojector} & CLIP-ViT-G/14 & Cross Attention & Vicuna-13B & MA+IA & 70.0 & - & - & - & - \\
    % InternLMXC2-4KHD & CLIP-ViT-L/14 & Partial LoRA & InternLM-XComposer2 & MA+IA & 90.0 & 68.6 & 81.0 & 77.2 \\
    
    LLaVA-OneVision-0.5B~\cite{li2024llava} & SigLIP & MLP & qwen2-0.5B & MA+IA & 70.0 & 41.8 & 61.4 & - & - \\
    LLaVA-OneVision-7B~\cite{li2024llava} & SigLIP & MLP & qwen2-7B & MA+IA & 87.5 & 68.8 & 80.0 & - & - \\
    Qwen2-VL-2B~\cite{wang2024qwen2vl} & CLIP-VIT-G/14 & Cross Attention & Qwen2-2B & MA+IA & 90.1 & 65.5 & 73.5 & 79.7 & 77.20 \\ 
    Qwen2-VL-7B~\cite{wang2024qwen2vl} & CLIP-VIT-G/14 & Cross Attention & Qwen2-7B & MA+IA & 94.5 & 76.5 & 83.0 & 84.3 & 84.58 \\ 
    DocVLM~\cite{nacson2024docvlmmakevlmefficient} & CLIP-ViT-G/14 + DocFormerV2 & Cross Attention & Qwen2-7B & MA+IA & 92.8 & 66.8 & - & 82.8 & - \\
    Qwen2-VL-72B~\cite{wang2024qwen2vl} & CLIP-VIT-G/14 & Cross Attention & Qwen2-72B & MA+IA & \cellcolor{gray!30}\textbf{96.5} & \cellcolor{gray!30}\textbf{84.5} & \cellcolor{gray!30}\textbf{88.3} & \cellcolor{gray!30}\textbf{85.5} & \cellcolor{gray!30}\textbf{88.70} \\ 

    DeepSeek-VL2-3B~\cite{wu2024deepseek} & SigLIP-SO400M-384 & Pixel-shuffle + MLP & DeepSeekMoE & MA+IA &88.9 &66.1 &81.0 &80.7 &79.18 \\
    DeepSeek-VL2-16B~\cite{wu2024deepseek} & SigLIP-SO400M-384 & Pixel-shuffle + MLP & DeepSeekMoE & MA+IA &92.3 &75.8 &84.5 &83.4 &84.00 \\
    DeepSeek-VL2-27B~\cite{wu2024deepseek} & SigLIP-SO400M-384 & Pixel-shuffle + MLP & DeepSeekMoE & MA+IA &93.3 &78.1 &86.0 &84.2 &85.40 \\
    
    Eagle2~\cite{li2025eagle2buildingposttraining} & SigLIP + ConvNeXt & MLP & Qwen2.5-7B & MA+IA & 92.6 & 77.2 & 86.4 & 83.0 & 84.80 \\
    \bottomrule
    \end{tabular}



%    InternVL 1.2, 1.5, 2.0.2.5, MPO
%TextHawk
%    Vary

 %   ocr-dependent: instructDoc, Cream, LayoutLLM,DocLLM

==> MLLM_OCR/Table/benchmark.tex <==
\scriptsize
    \begin{tabular}{cccccccc}
    \toprule
    Types & Benchmark & Language &\#Scenario & \#Task & \#Num & \#Instruction &Open-source  \\
    \midrule
    \multirow{3}{*}{Document} 
    & OCREval~\cite{lv2023kosmos} & English & Multi-domain & 1 & 2,297 & - & \ding{51}\\
    & MMLongBench-Doc~\cite{Ma2024NEURIPS_MMLongBench_Doc_Benchmarking} & English & Multi-domain Long Documents & 3 & 135 & 1k & \ding{51}\\
    & Do-GOOD~\cite{He2023ARXIV_Do_GOOD_Towards} & English & Industry document  & 3 & 410k & 50k & \ding{51}\\
    \midrule 
    \multirow{4}{*}{Chart }& ChartY~\cite{chen2024onechart} & English,Chinese & Charts and Plots  & 1 & 6k & 6k & \ding{51}\\
    & ChartX~\cite{xia2024chartx} & English & Charts and Plots & 7 & 6k & 6k & \ding{51}\\
    & MMC~\cite{Liu2024NAACL_MMC_Advancing_Multimodal} & English & Plots (Real world data source) & 9 & 1.7k& 2.9k & \ding{55}\\
    & ChartBench~\cite{Xu2024ARXIV_ChartBench_A_Benchmark} & English & Plots (Real world data source) & 2 & 68k& 549k & \ding{55}\\
    \midrule  
    \multirow{3}{*}{Table} & TableVQA-Bench~\cite{Kim2024ARXIV_TableVQA_Bench_A} & English & Scientific and Financial Reports & 3 & 0.9k & 1.5k & \ding{51}\\
    & MMTab-eval~\cite{zheng2024multimodal} & English & Scientific and Financial Reports & 9 & 23k & 49k & \ding{51}\\
    & ComTQA~\cite{Zhao2024NEURIPS_TabPedia_Towards_Comprehensive} & English & Scientific and Financial Reports & 4 & 1.6k & 9k & \ding{51}\\
    \midrule 
    \multirow{1}{*}{GUI} 
    & Screen2Words~\cite{wang2021screen2words} & English & Android app screenshot & 1 & 22k & 112k & \ding{51}\\
    \midrule 
    \multirow{8}{*}{Synthesis} & OCRbench~\cite{liu2024ocrbench} & English & Multi-domain & 5 & 0.9k & 1k & \ding{51}\\
    & Seed-bench-2-plus~\cite{li2024seed} & English & Multi-domain & 1 & 0.6k & 2.3k & \ding{51}\\
    & CONTEXTUAL~\cite{wadhawan2024contextual} & English & Multi-domain & 1 & 0.5k & 0.5k & \ding{51}\\
    & OCRBench v2~\cite{fu2024ocrbench} & English & Multi-domain & 23 & 9.5k & 10k & \ding{51}\\
    & FOX~\cite{liu2024focus} & English,Chinese & Academic Document Corpus & 9 & 0.7k & 2.2k & \ding{51}\\
    & DocLocal4K~\cite{hu-etal-2024-mplug} & English & Multi-domain & 2 & 4.2k & 4.2k & \ding{51}\\
    & CC-OCR~\cite{yang2024cc} & Multilingual & Multi-domain & 3 & 7k & - & \ding{51}\\
    & MMDocBench~\cite{Zhu2024ARXIV_MMDocBench_Benchmarking_Large} & English & Multi-domain & 15 & 2.4k & 4.3k & \ding{51}\\
    
    \bottomrule
    \end{tabular}

==> MLLM_OCR/Table/dataset.tex <==
\scriptsize
    \begin{tabular}{llccccc}
    \toprule
    Types & Dataset & Language & Scene Sources & \#Images & \#Q\&A pairs & Answer in Picture \\
    \midrule
    \multirow{4}{*}{Document} & DocVQA~\cite{mathew2021docvqa} & English & Industry document & 12,767&  50,000 & Yes\\
    & Docmatix~\cite{laurenccon2024building} & English & Industry document & 2.4M & 9.5M & Yes\\
    & InfoVQA~\cite{mathew2022infographicvqa} & English & Infographics & 5,485 & 30,035 & Yes\\
    & MP-DocVQA~\cite{tito2023hierarchical} & English & Industry documents & 47,952 & 46,176 & Yes\\
    &DocGenome~\cite{xia2024docgenome} & English & Scientific document & 6.8M & 3,000 & Yes\\
    &IIT-CDIP~\cite{xu2020layoutlm} & English & Multi-domain & 11M & - & -\\
    &synthdog~\cite{kim2022ocr}& English & Multi-domain & 2M & - & -\\
    &CCPdf~\cite{turski2023ccpdf}& Multiple languages & Multi-domain & 1.1M & - & - \\
    \midrule 
    \multirow{4}{*}{Chart }& ChartQA~\cite{masry2022chartqa} & English & Charts and Plots  & 20,882 & 32,719 & Yes\\
    & PlotQA~\cite{methani2020plotqa} & English & Plots (Real world data source) & 224,377 & 28.9M & Yes\\
    & FigureQA~\cite{kahou2017figureqa} & English & Science style image & over 100,000 & over 1.3M& Yes\\
    & DVQA~\cite{kafle2018dvqa} & English & Data Visualizations & 300,000 & 3,487,194 & Yes\\
    \midrule 
    \multirow{4}{*}{Scene} & TextCaps~\cite{sidorov2020textcaps} & English & Scene Text (Open Images) & 28,408 & 142,040 & Yes\\
    & TextVQA~\cite{singh2019towards} & English & Scene Text (Open Images) & 28,408 & 45,336 & Yes\\
    & ST-VQA~\cite{biten2019scene} & English & Scene Text & 23,038 & 31,791 & Yes\\
    & MT-VQA~\cite{wen2024mt} & Multiple languages & 20 fine-grained scenes & 8,794 & 28,607 & Yes\\
    \midrule 
    \multirow{1}{*}{Table} & TableQA~\cite{sun2020tableqa} & English & Financial reports & 6,000 & 64,891 & Yes\\
    &WikiTableQuestions~\cite{pasupat2015compositional}& English & Multi-domain & 2,108 & 22,033 & Yes\\
    &DeepForm~\cite{svetlichnaya2020deepform}& English & Political campaign finance receipts & 20,000 & - & - \\
    \midrule 
    \multirow{2}{*}{Math} & GeoQA~\cite{chen2021geoqa} & Chinese & Mathematics test questions & 5,010 & 5,010 & No\\
    & GeoQA+~\cite{cao2022augmented} & Chinese & Online education website & 12,054 & 12,054 & No\\
    % \midrule 
    % \multirow{1}{*}{Code}&&&&&&\\
    % &&&&&&\\
    \midrule 
    \multirow{2}{*}{GUI} & ScreenQA~\cite{hsiao2022screenqa} & English & Mobile app screenshots & 35,352 & 85,984 & Yes\\
    & Screen2Words~\cite{wang2021screen2words} & English & Android app screenshot & 22,417 & 112,085 & No\\
    \bottomrule
    \end{tabular}



==> MLLM_OCR/sec/0_abstract.tex <==
\begin{abstract}
The recent emergence of Multi-modal Large Language Models (MLLMs) has introduced a new dimension to the Text-rich Image Understanding (TIU) field, with models demonstrating impressive and inspiring performance. However, their rapid evolution and widespread adoption have made it increasingly challenging to keep up with the latest advancements. To address this, we present a systematic and comprehensive survey to facilitate further research on TIU MLLMs. Initially, we outline the timeline, architecture, and pipeline of nearly all TIU MLLMs. Then, we review the performance of selected models on mainstream benchmarks. Finally, we explore promising directions, challenges, and limitations within the field.
% LLM-based text-rich image understanding models, through joint vision-language modeling, overcome modality bias and enhance zero-shot capabilities, significantly advancing the comprehension of text-rich images and establishing a new research paradigm. This paper systematically reviews the progress of multimodal large language models (MLLMs) in the TIU domain, analyzing design paradigms of model architectures, training methodologies, datasets, and performance benchmarks. It identifies future challenges and provides theoretical foundations and practical pathways for developing universal TIU models.

\end{abstract}
% \begin{IEEEkeywords}
% Document Understanding, Multimodal Large Language Model, Survey.
% \end{IEEEkeywords}

==> MLLM_OCR/sec/1_intro.tex <==
\section{Introduction}

% 介绍Ttext-rich image 及TIU 任务，引出基于LLM 的方法近期发展迅猛，急需一篇综述来介绍相关的进展


%Historically, perception and understanding tasks were handled separately through specialized models or multi-stage pipelines. Recent advances in vision-language models have unified these capabilities under Visual Question Answering (VQA) frameworks, driving research toward end-to-end universal models. As shown in Figure 1, the emergence of large language models (LLMs) marks a paradigm shift. Pre-LLM approaches like LayoutLM \cite{Xu2019ARXIV_LayoutLM_Pre_training} and Donut relied on self-supervised pre-training (masked language modeling, layout prediction) or OCR-aware tasks (text recognition, order recovery), followed by task-specific fine-tuning. While effective in controlled settings, these methods exhibit limited zero-shot generalization.

Text-rich images play a pivotal role in real-world scenarios by efficiently conveying complex information and improving accessibility \cite{biten2019scene}. Accurately interpreting these images is essential for automating information extraction, advancing AI systems, and optimizing user interactions. To formalize this research domain, we term it \textbf{T}ext-rich \textbf{I}mage \textbf{U}nderstanding (\textbf{TIU}), which encompasses two core capabilities: perception and understanding. The perception dimension focuses on visual recognition tasks, such as text detection \cite{liao2022real}, text recognition~\cite{guan2025ccdplus}, formula recognition \cite{TRUONG2024110531, guan2024posformer}, and document layout analysis \cite{Yupan2022ARXIV_LayoutLMv3_Pre_training}. The understanding dimension, conversely, requires semantic reasoning for applications like key information extraction and document-based visual question answering (\emph{e.g.}, DocVQA \cite{mathew2021docvqa}, ChartQA \cite{masry2022chartqa}, and TextVQA~\cite{singh2019towards}).

Historically, perception and understanding tasks were handled separately through specialized models or multi-stage pipelines. Recent advances in vision-language models have unified these tasks within Visual Question Answering (VQA) paradigms, driving research towards the development of end-to-end universal models.


Figure \ref{fig:Development} presents an evolutionary timeline delineating critical milestones in unified text-rich image understanding models. The trajectory reveals two distinct eras: (a) The pre-LLM period (2019-2022) characterized by specialized architectures like LayoutLM \cite{Xu2019ARXIV_LayoutLM_Pre_training} and Donut \cite{Kim2021SEMANTIC_Donut_Document_Understanding}, which employed modality-specific pre-training objectives (masked language modeling, masked image modeling, \textit{etc.}) coupled with OCR-derived supervision (text recognition, spatial order recovery, \textit{etc.}). While effective in controlled settings, these models exhibited limited adaptability to open-domain scenarios due to their task-specific fine-tuning requirements and constrained cross-modal interaction mechanisms. (b) The post-LLM era (2023–present) is marked by the growing popularity of LLMs. Some studies propose Multimodal Large Language Models (MLLMs), which integrate LLM with visual encoders to jointly process visual tokens and linguistic elements through unified attention mechanisms, achieving end-to-end sequence modeling.
% In the following sections of this paper, such large models will be uniformly referred to as MLLMs.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/2.pdf} 
    \vspace{-2em}
    \caption{The general model architecture of MLLMs and the implementation choices for each component.} 
    \label{fig:Architecture} 
    \vspace{-1em}
\end{figure*}

This paradigm evolution addresses two critical limitations of earlier methods. First, the emergent MLLM framework eliminates modality-specific inductive biases through homogeneous token representation, enabling seamless multi-task integration. Second, the linguistic priors encoded in LLMs empower unprecedented zero-shot generalization and allow direct application to diverse tasks without task-specific tuning. 

% \textcolor{red}{Whether general-purpose MLLMs or TIU-specific models}, 
Although these MLLMs present impressive and inspiring results, their rapid evolution and broad adoption have made tracking cutting-edge advancements increasingly challenging. Therefore, a systematic review that is tailored for documents to summarize and analyse these methods is in demand. However, 
existing surveys on text-rich image understanding often exhibit narrow focus: they either analyze domain-specific scenarios (e.g., tables and figures \cite{huang2024detection}, charts \cite{Huang2024ARXIV_From_Pixels_to, alshetairy2024transformersutilizationchartunderstanding}, forms \cite{abdallah2024transformers}) or emphasize unified deep learning frameworks \cite{subramani2011survey,ding2024deep}.

Our systematic survey addresses the gap by providing the first comprehensive analysis of nearly all TIU MLLMs in four dimensions: Model Architectures (Section \ref{sec:model_architecture}), Training Pipeline  (Section \ref{sec:training_pipeline}), Datasets and Benchmarks (Section \ref{sec:datasets}), Challenges and Trends (Section \ref{sec:summary}). This holds both academic and practical significance for advancing the field.



%To systematically establish a research framework for TIU MLLMs, we outline its design framework through the following two aspects: Model Architecture \ref{sec:model_architecture}), Training Pipeline (Section \ref{sec:training_pipeline}). Section \ref{sec:datasets} organizes mainstream datasets and benchmarks for training and evaluation. Finally, Section \ref{sec:summary} synthesizes key insights, identifies unresolved challenges, and proposes research directions to inspire the design of more powerful TIU MLLMs.

% We decompose the general model architecture into three core components: Visual Encoder (Section \ref{section_visual_encoder}), Modality Connector (Section \ref{section_connector}), and LLM Decoder (Section 2.3).
% The training pipeline elaborates on the current mainstream alignment methods, primarily consisting of three stages: Modality Alignment (i.e. Pre-training) (Section 3.1), Instruction Alignment (i.e. Fine-tuning) (Section 3.2), and Preference Alignment (i.e. Post-training) (Section 3.3). Among these, Pre-training and Fine-tuning are essential, while Post-training is optional. 
%Subsequently, in Section 4, we summarize the mainstream datasets used for pre-training and fine-tuning. In Section 5, we comprehensively review the mainstream benchmarks and the performance of major LLM-based TIU models on these benchmarks. In Section 6, we conclude the paper by summarizing the key points, highlighting existing challenges, and proposing potential research directions. We hope that this survey will help researchers gain a deeper understanding of the field and inspire the design of more efficient LLM-based TIU models.

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Figure/3.pdf}
    \vspace{-1em}
    \captionof{figure}{The evolutionary tree of modern LLMs traces the development of language models in recent years and highlights some of the most well-known models. According to the classification of Encoders, the \textcolor[HTML]{2E54A1}{blue} branch is ocr-free, the \textcolor[HTML]{C81D31}{pink} branch is ocr-based, and the \textcolor[HTML]{588F32}{green} branch is Mixture of Encoders.}
    \label{fig:2}
    \vspace{-1em}
\end{figure*}

==> MLLM_OCR/sec/2_method.tex <==
\section{Model Architecture}
\label{sec:model_architecture}
%VDU任务详细介绍：1.答案在图上；2.答案不在图上；及公共数据集

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figure/Architecture.png} 
%     \caption{The general model architecture of MLLMs and the implementation choices for each component} 
%     \label{fig:Architecture} 
% \end{figure*}


TIU MLLM methods typically leverage pre-trained general visual foundation models to extract robust visual features or employ OCR engines to capture text and layout information from images. A modality connector is then used to align these visual features with the semantic space of the language features from the LLM. Finally, the combined visual-language features are fed into the LLM, which utilizes its powerful comprehension capabilities for semantic reasoning to generate the final answer.
As illustrated in Figure~\ref{fig:Architecture}, the framework of TIU MLLMs can be abstracted into three core components: Visual Encoder, Modality Connector, and LLM Decoder. 
% In the subsequent sections, we systematically analyze the implementation choices and technical considerations for each component.


%Multi-modal Document Understanding aims to extract meaningful information from text images of various types, such as charts, tables, documents, and other scene texts, through a question-driven image-to-sequence task.
%Some early studies~\cite{yang2021tap} have explored end-to-end solutions within a specialist model, which may not provide broad robustness and generality for various scenarios.
%The recent emergence of Multi-modal Large Language Models (MLLMs) has introduced a novel dimension to the field by linking visual image tokens and language tokens in a sequence-to-sequence format, thereby facilitating task unification. This structure seamlessly integrates computer vision with natural language processing, allowing MLLMs to significantly enhance text reading capabilities, supported by large-scale data and GPU resources. These methods can be roughly categorized into two types: OCR-dependent MLLMs~\cite{lu2024bounding,lee2025moai,luo2022bi,Instructdoc,Doclayllm} and OCR-free MLLMs~\cite{internvl,minigpt,MiNi-Monkey,Monkey,Mplug-Docowl2,UReader}.
%A Bounding Box is Worth One Token:Interleaving Layout and Text in a Large Language Model for Document Understanding
\subsection{Visual Encoder}
\label{section_visual_encoder}
The Visual Encoder $\mathcal{F}(\cdot)$ is responsible for transforming input image $\mathbf{I}$ into feature representations $\mathbf{V}$, expressed as $\mathbf{V} = \mathcal{F}(\cdot)(\mathbf{I})$. As illustrated in Figure \ref{fig:2}, these encoders can be categorized into OCR-free, OCR-based, or a hybrid approach.
% \begin{equation}
%     \begin{aligned}
%         \mathbf{F} = \mathcal{F}(\cdot)(\mathbf{I})
%     \end{aligned}
% \end{equation}
% Depending on the task requirements, the Visual Encoder can be implemented in various forms, including: OCR-free encoder, OCR-based encoder, or a mixture of encoders. 
% \textcolor{red}{Below is a summary of common types of Visual Encoders and their characteristics:}



\noindent \textbf{OCR-free Encoder} is widely used to extract high-level visual features, effectively capturing essential information about objects, scenes, and textures. The commonly used OCR-free encoders include (1) \textbf{CLIP} \cite{radford2021CLIP}; (2) \textbf{ConvNeXt} \cite{woo2023convnext}; (3) \textbf{SAM} \cite{kirillov2023SAM}; (4) \textbf{DINOv2} \cite{oquab2023dinov2}; (5) \textbf{Swin-T} \cite{liu2021swin}; (6) \textbf{InternViT} \cite{chen2024internvlscalingvisionfoundation}.

% 1) \textbf{CLIP-ViT} \cite{radford2021CLIP}, excels in vision-language alignment, making it well-suited for processing global semantic information; 

% 2) \textbf{ConvNeXt} \cite{woo2023convnext}, performs exceptionally well in visual tasks, making it ideal for extracting local detailed features; 

% 3) \textbf{SAM} \cite{kirillov2023SAM}, focuses on image segmentation, providing precise object boundary details;

% 4) \textbf{DINOv2} \cite{oquab2023dinov2}, with its self-supervised learning capabilities, is highly effective in capturing rich and robust visual representations across diverse tasks; 

% 5) \textbf{SwinTransformer}, known for its hierarchical architecture and shifted window mechanism, excels in handling high-resolution images and capturing multi-scale features, making it a powerful choice for tasks requiring detailed spatial understanding; 

% 6) \textbf{InternViT}, achieves direct alignment with LLMs during training, enabling it to exhibit superior adaptability and performance in multimodal tasks compared to other ViT models.

\noindent \textbf{OCR-based Encoder} processes textual content and layout information from OCR outputs through three primary paradigms:
(1) \textbf{Direct Input} injects raw OCR texts into LLMs, though long sequences degrade inference efficiency \cite{he2023icl};
(2) \textbf{Cross-Attention} dynamically selects salient content via attention mechanisms within LLMs \cite{Wang2023ARXIV_DocLLM_A_layout};
(3) \textbf{External Encoder} employs specialized models like BLIP-2~\cite{li2023blip2bootstrappinglanguageimagepretraining}, DocFormerv2~\cite{nacson2024docvlmmakevlmefficient} or LayoutLMv3~\cite{Yupan2022ARXIV_LayoutLMv3_Pre_training} to structure OCR features before LLM integration \cite{ Tanaka2024AAAI_InstructDoc_A_Dataset, Luo2024CVPR_LayoutLLM_Layout_Instruction, Fujitake2024LREC_LayoutLLM_Large_Language}.

\noindent \textbf{Mixture of Encoders} strategies address TIU task complexity through two dominant configurations:
(1) \textbf{Dual OCR-Free} architectures (\emph{e.g.}, CLIP+SAM) combine complementary visual encoders to jointly capture global semantics and local details~\cite{wei2024vary};
(2) \textbf{Hybrid OCR-Free/OCR-Based} systems (\emph{e.g.}, CLIP+LayoutLMv3) synergize visual feature extraction with text-layout understanding, proving particularly effective for document-level tasks requiring multimodal reasoning \cite{Liao2024ARXIV_DocLayLLM_An_Efficient}.

\begin{comment}
\noindent \textbf{OCR-Based Encoder} is designed to efficiently encode textual content and layout information extracted by the OCR engine, thereby providing robust support for subsequent semantic understanding tasks. The forms of OCR encoders can be summarized as follows:

1) \textbf{Direct Input}: This approach inputs OCR texts or layouts into the LLM directly, which results in excessively long input lengths, adversely affecting inference speed and model performance.
%%%previous version
% Directly inputs the OCR texts into the LLM, or models document layouts by inserting spaces and newline characters between OCR-recognized text lines, providing the LLM with input that includes basic layout information. However, a significant drawback is that the input length may become excessively long, which can negatively impact inference speed and model performance.

2) \textbf{Cross-Attention}: This approach selects important contents from OCR engine outputs by a cross-attention mechanism within the LLM.
%%%previous version
% Through a cross-attention mechanism, the interaction between OCR positional information and text features is achieved within the LLM. This approach alters the internal structure of the LLM, potentially affecting its generality and generalizability.

3) \textbf{External Encoder}: \textcolor{red}{Utilizes BLIP-2 or LayoutLMv3 to encode document OCR information, which is then fed into the LLM.} 
% It avoids the issue of excessively long inputs and enhances information density. However it requires additional encoders, and understanding capability of these encoders may not match that of the LLM, necessitating significant training resources for alignment.


\noindent \textbf{Mixture of Encoders}
The inspiration for using a mixture of encoders stems from the complexity and diversity of TIU tasks. While single visual encoders excel in specific tasks, they often struggle to balance the capture of global and local information when faced with high-resolution images, complex scenes, or multitask learning. 
% Given the theoretically vast number of possible combinations, only the mainstream mixture strategies in LLM-based TIU tasks are listed here:
Here, we outline the mainstream mixture strategies used in LLM-based TIU tasks:

1) \textbf{Dual OCR-Free Encoders}. This approach combines two OCR-free encoders, where one excels at processing low-resolution inputs and the other specializes in high-resolution inputs, such as CLIP paired with SAM. By leveraging their complementary strengths, this integration enables the model to capture both global semantic information and detailed local features, significantly enhancing its ability to handle complex visual tasks.

%%%previous version
% This approach combines two OCR-free encoders, designed with the rationale that one excels at processing low-resolution inputs while the other specializes in high-resolution inputs, such as CLIP and ConvNeXt, or CLIP and SAM. By leveraging their complementary strengths in extracting high-level visual features, the integration of these encoders enables the model to simultaneously capture global semantic information and fine-grained local details, thereby significantly enhancing its capability to handle complex visual tasks.

2) \textbf{Hybrid of OCR-Free and OCR-Based Encoders}. This strategy combines an OCR-free encoder (e.g., CLIP) with an OCR-based encoder to simultaneously process visual and textual information. OCR-free encoders focus on extracting high-level visual features, such as objects and scenes, while OCR-based encoders specialize in capturing textual content and layout information from images. This hybrid approach is particularly effective for tasks involving text-rich images or documents.
\end{comment}

\subsection{Modality Connector}
\label{section_connector}

Visual embeddings $\mathbf{V} = [\mathbf{v}_{1}, \mathbf{v}_{2},..., \mathbf{v}_{n}]$ and language embeddings $\mathbf{T} = [\mathbf{t}_{1}, \mathbf{t}_{2},..., \mathbf{t}_{l}]$ belong to different modalities. Consequently, to bridge the gap between them and create unified sequence representations that can be processed by large language models (LLMs), a modality connector $\xi: \mathbf{V} \xrightarrow{} \mathbf{T}$ is typically employed, which is responsible for converting $n$ visual features into $m$ visual tokens.
We review the strategies previously utilized in the literature for this purpose. 

Specifically, the modality connector can be easily implemented using a simple linear projector or multi-layer perception (MLP), \emph{i.e.,} $m=n$, but faces challenges in scalability and efficiency. Recent works also proposed more effective and innovative modality connectors from various perspectives, such as token compression and token reduction. The former focuses on reducing the number of inputs to the MLLM token with lossless compression, and the latter addresses the issue of costly tokens by removing redundant and unimportant token representations, such as background tokens.

\noindent \textbf{Token Compression}

1) Pixel shuffle \cite{chen2024far} rearranges the elements of a high-resolution feature map $(h, w)$ to form a lower-resolution feature map $(\frac{h}{s}, \frac{w}{s})$ by redistributing the spatial dimensions into the depth (channels) of the feature map. Here, $s$ denotes the compression rate. 
% This operation effectively reduces the features' width and height, while increasing the number of channels. Specifically, pixel shuffle typically has two variations: image-level shuffle and window-level shuffle. The former divides the entire feature map into $s\times s$ parts and concatenates each part $(\frac{h}{s}, \frac{w}{s})$ along the channel dimension. In contrast, similar to the Swin Transformer, the window-level shuffle performs the shuffle process within each window of size  $s\times s$ and concatenates the shuffled features along the spatial dimension.
We summarized the process as $\xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{\frac{h}{s} \times \frac{w}{s} \times (s\times C)}$.
% \begin{equation}
%     \xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{\frac{h}{s} \times \frac{w}{s} \times (s\times C)}
% \end{equation}

% 2) Cross-attention used in \cite{bai2023qwenvlversatilevisionlanguagemodel} operates on the queries which are a group of trainable vectors and the keys which are the image features produced by the vision encoder. 
% \begin{equation}
%     \xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{q \times D}
% \end{equation}

\noindent \textbf{Token Reducer} 

1) Cross Attention \cite{alayrac2022flamingovisuallanguagemodel,li2023blip2bootstrappinglanguageimagepretraining,chen2024internvlscalingvisionfoundation,dai2023instructblipgeneralpurposevisionlanguagemodels} operates on the queries (a group of trainable vectors or the key features of the model itself) and the keys which are the image features produced by the vision encoder. We summarized the process as $\xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{q \times D}$. 
% \begin{equation}
%     \xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{q \times D}
% \end{equation}


% introduces a set of custom-defined learnable embeddings that serve as adaptive filters to selectively extract valuable information from image embeddings relevant to the task. Specifically, several cross-attention layers are applied to facilitate this process, where these learnable embeddings act as the query, while the image embeddings serve as the key and value. In MLLMs, the number $q$ of learnable embeddings is typically set to a value significantly lower than the total number of image embeddings. We summarized the process as follows:
% \begin{gather}
%     \xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{q \times D}
% \end{gather}

2) H-Reducer~\cite{Hu2024ARXIV_mPLUG_DocOwl_1} introduces the $1 \times 4$ convolution layer to reduce visual features, as the horizontal texts are widely found in natural scenes and semantically coherent.
% consists of a convolution layer and a fully connected linear layer. The convolution kernel is set to $1 \times 4$, as the horizontal texts are widely found in natural scenes and semantically coherent. Then, a fully connected layer is used to align reduced visual features to the language embedding space $\mathbb{R}^{D}$. 
We summarized the process as $\xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{h \times \frac{w}{4} \times D}$.
% \begin{gather}
%     \xi: \mathbb{R}^{h \times w \times C} \xrightarrow{} \mathbb{R}^{h \times \frac{w}{4} \times D}
% \end{gather}

3) C/D-abstract~\cite{cha2024honeybee} employs Convolution and Deformable Attention respectively to achieve both flexibility and locality preservation.

4) Attention Pooling~\cite{Liu2024ARXIV_TextMonkey_An_OCR,Huang2024ARXIV_Mini_Monkey_Alleviating} identifies important tokens and removes redundant ones. To evaluate the redundancy of image features, the similarity between image tokens is often utilized~\cite{Liu2024ARXIV_TextMonkey_An_OCR}. This method selects tokens that are highly unique and lack closely similar counterparts. Average pooling is the most special one.
\begin{table*}[!t]
    \centering
    \scalebox{0.78}{
    \input{Table/MLLM}
    }
    \vspace{-0.5em}
    \caption{The summary of representative mainstream MLLMs, including the model architectures, training pipelines, and scores on the four most popular benchmarks of TIU. ``Private'' indicates that the MLLM utilizes a proprietary large model. ``$\dagger$'' indicates the results are obtained by downloading official open-source model and testing it locally.}
    \label{tab:mllm_summary}
    \vspace{-1.5em}
\end{table*}

\subsection{LLM Decoder}
% The LLM decoder receives the aligned features from the Modality Connector, integrates them into the language context for reasoning, and generates the final output based on specific task requirements, such as text answers, image descriptions, structured data, and more.
The aligned features are fed into the LLM decoder together with the language embeddings for reasoning. We list the commonly used LLMs in MLLM:
% Below, we outline the commonly used LLMs in MLLMs: %, along with their key characteristics:

\noindent \textbf{LLaMA Series}. LLaMA \cite{touvron2023llama, touvron2023llama2, dubey2024llama} is a series of open-source large language models developed by Meta, aimed at promoting openness and innovation in artificial intelligence technology, LLaMA series include models of varying parameter scales (e.g., 7B, 13B, 34B). 
% Since the release of the first-generation model LLaMA 1 in 2023, the series has undergone continuous iterative upgrades in terms of parameter scale, training data, context window, and multimodal capabilities. The latest LLaMA 3.2 supports a context length of 128K tokens.

\noindent \textbf{Qwen Series}. Qwen \cite{bai2023qwen,yang2024qwen2}, developed by Alibaba, is a multilingual LLM that supports both Chinese and English.
%Qwen-VL, its multimodal variant, enables joint understanding and generation of images and text.
% Since its initial release in 2023, the Qwen series of models has become a significant force in the field of large models through continuous technological innovation and open-source strategies. The latest version of this series is Qwen2.5, which supports a context window of up to 1M tokens and demonstrates exceptional performance in reasoning tasks. Multimodal models based on Qwen, such as Qwen-VL \cite{bai2023qwenvl} and Qwen2-VL \cite{wang2024qwen2}, have also shown immense potential in the field of TIU.


\noindent \textbf{Vicuna Series}. Vicuna \cite{zheng2023judging} is an open-source large language model built on LLaMA, developed by research teams from institutions including UC Berkeley, CMU, and Stanford. 
% It is offered in two parameter sizes: 7B and 13B. The Vicuna series has multiple versions, with the widely used Vicuna-v1.5 version supporting context lengths of 4K and 16K tokens. Since the acclaimed open-source multimodal large language model LLaVA \cite{liu2024visual, liu2024improved} adopted Vicuna as its LLM backbone, numerous TIU models have been enhanced based on LLaVA. This has significantly advanced the development of LLM-based TIU methods.


\noindent \textbf{InternLM series}. InternLM \cite{cai2024internlm2} is an open-source large language model series developed by the Shanghai Artificial Intelligence Laboratory, with the latest version, InternLM 2.5, offering parameter sizes of 1.8B, 7B, and 20B. 
% As a bilingual model, it supports both Chinese and English, making it versatile for a wide range of applications. A key highlight of InternLM is its ability to handle a 1M (1 million) token context window, which makes it particularly effective for tasks involving long-text processing, such as document comprehension and multi-turn dialogue.






% \subsection{OCR-dependent MLLMs} 
% They enhance document understanding by integrating text, layout, and other data extracted from external OCR tools~\cite{PP-OCRv3} into large language models. LayTextLLM~\cite{LayTextLLM} and DocLayLLM~\cite{Doclayllm} both utilize an external OCR engine to extract layout and text, integrating them into a LLM for document understanding. However, this integration complicates the workflow and leads to an excess of auxiliary tokens, particularly in images with dense texts.

% \noindent \textbf{Document encoder}

% \noindent \textbf{CoT}

% \noindent \textbf{Ocr output as context}

% % 这段应该结合 intro 里对当前方法的批评，再次强调当前的方法缺少spatially-aware alignment
% \subsection{OCR-free MLLMs} 
% These methods perform the multi-modal document understanding task by directly producing question-driven outputs in an end-to-end manner. These methods typically focus on high-resolution image processing~\cite{Monkey,UReader,mplug-docowl1.5,docpedia}, efficient token compression~\cite{zhang2024token,Mplug-Docowl2,yu2024texthawk2}, and refined attention mechanisms~\cite{MiNi-Monkey,VisualCoT}. 

% \noindent \textbf{High resolution}

% \noindent \textbf{Visual encoder alignment}

% \noindent \textbf{Token compresssion}


% \subsection{Vision Language Pre-training}
% Inspired by recent advancements~\cite{CLIP,DINO,SigLIP,SIGA,SAM} in pre-training techniques, the integration of image and text multi-modal information into OCR-related tasks has gained increasing attention. Using cross-modal visual-language priors, early works focused on endowing visual foundation models with semantic knowledge~\cite{FastTCM,TCM,SKTM,VLPT,oCLIP,duan2024odm,guan2025bridging,CCD} for applications such as text spotting, detection, recognition, removal, and super-resolution. As MLLMs rapidly develop, researchers are further capitalizing on these visual-language priors to bridge visual and language modalities through diverse pre-training tasks~\cite{UReader,Cream,Doclayllm,DocLLM,docpedia,LayTextLLM,internvl,liu2024textmonkey,minigpt,mplug-docowl1.5}. For instance, UReader~\cite{UReader} introduces the Read Full Text (RFT) task in VQA form for enhancing document-level understanding. Park \emph{et al.}~\cite{parkhierarchical} propose two new pretext tasks: Reading Partial Text (RPT) and Predicting Text Position (PTP). Similarly, KOSMOS-2.5~\cite{lv2023kosmos} designs a Visual Text Grounding (VTG) task, which inputs the texts within images and produces the corresponding bounding boxes. mPLUG-DocOWL~\cite{mplug-docowl1.5} integrates multiple tasks to conduct the struct-aware parsing in documents, tables, charts, and natural scenes. However, these question-driven image-to-sequence tasks predominantly emphasize \emph{semantic alignment}, and may rely on the powerful semantic context capabilities of LLMs when responding. Following these VQA forms, we further introduce an additional mask generation pre-text task (VQAMask) to explicitly facilitate spatially-aware visual-language alignment.

==> MLLM_OCR/sec/3_training.tex <==
\section{Training Pipeline}
\label{sec:training_pipeline}
The training pipeline of MLLM for TIU can be delineated into three main stages: 1) Modality Alignment (\textbf{MA}); 2) Instruction Alignment (\textbf{IA}); and 3) Preference Alignment ({\textbf{PA}}).

\subsection{Modality Alignment}
In this stage, previous works typically use OCR data from traditional OCR tasks~\cite{guan2024bridging,guan2023ccd} to pre-train the MLLM, which aims to bridge the modality gap. The general alignment methods can be categorized into three types: recognition, localization, and parsing.

\noindent \textbf{Read Full Text.} UReader~\cite{ye2023ureader} is the first to explore unified document-level understanding, which introduces the Read Full Text task in VQA for pre-training. Specifically, they include 1) reading all texts from top to bottom and left to right, and 2) reading the remaining texts based on given texts.
% UReader leverages text and positional information from images to organize the text in a common reading order: from top to bottom and left to right. There are two approaches to reading the entire text: one is to start from the beginning and read the complete text, and the other is to set a starting point, provide the text to the left of this starting point, and require the model to continue reading from there. For example, an instruction to start reading from the beginning could be ''Recognize the text in the image.'' An instruction to continue reading might be ''The words on this image are {left text}. Continue reading the text.''
Compared to reading the full text, some works~\cite{Lv2024ARXIV_KOSMOS_2_5, Hu2024ARXIV_mPLUG_DocOwl_1} proposes a more structured reading approach by predicting the image markdown, not text transcriptions.
% transcribing the text transcriptions into Markdown format. This approach provides richer structural information for document understanding. For example, $<s><image>Image Embedding</image><md>[Markdown Text]</s>$. Additionally, KOSMOS-2.5 generates the coordinates for each line of text, with each text block being assigned its spatial coordinates in the image, represented as $<s><image>Image Embedding</image><ocr>{\cup}_{n=1}^{N}(B_n \oplus T_n) </s>$, with $\oplus$ indicating the alignment of text lines$T_n$ with their corresponding coordinate bounding boxes$B_n$.Notably, the two tasks are distinguished using <ocr> and <md> in the prompt.

\noindent \textbf{Reading Partial Text within Localization.} Due to the length of document texts, instructions for reading the full text may risk truncation because of the limited token length in LLMs. To address these limitations, Park \emph{et al.}\cite{park2024hierarchical} introduced two novel tasks: Reading Partial Text (RPT) and Predicting Text Position (PTP). The former randomly selects and reads continuous portions of text in the reading order from top to bottom and left to right. For example, ``Q: What is the text in the image between the first 30\%, from 20\% to 40\%, or the last 16\%?'' For the PTP task, given a text segment, the MLLM aims to infer its relative position (percentage format) within the full text. 
% Notably, the relative position here refers to the percentage of the entire text that the segment occupies. 
For example, ``Q: Where is the text {query texts} located within the image? A: 40\% to 80\%''.
% \noindent \textbf{Location.} The aforementioned method by Park et al. uses percentage-based positioning to help LLMs enhance their understanding of the layout of visual text. 
However, this approach can be somewhat obscure and challenging to express accurately. 

Alternatively, some methods~\cite{hu2024mplug_docowl1.5_arxiv,yu2024texthawk,liu2024hrvda} extract texts based on specific spatial positions, which are summarized into two types.
% In addition, extracting text using specific positional information is also a popular method for instruction fine-tuning. The specific methods can be divided into the following two approaches: 
1) Text Recognition aims to extract the textual content from a given position in the image, ensuring that the model can accurately recognize and extract text within specific regions.
2) Text Grounding involves identifying the corresponding bounding box for specific text in the image, which assists the model in understanding the document layout.

% matching specific text in the image with image regions to identify the corresponding bounding box, helping the model understand the layout of text within the visual scene.

% Due to the varying dimensions of each image, the same region may present different coordinate values after image processing, which is disadvantageous for model learning. Researchers typically normalize the representation of bounding boxes, transforming each continuous value within the bounding box into a discrete position label, such as a range from 0 to 999. For example, DocOWL has designed two complementary localization tasks: Multi-grained Text Grounding and Multi-grained Text Recognition. These tasks define four granularities of text: word, phrase, line, and block. A ''word'' indicates a bounding box containing only a single word, a ''phrase'' consists of multiple adjacent words, a ''line'' is composed of a horizontal line of text, and a ''block'' is a combination of multiple consecutive lines.

\noindent \textbf{Parsing.} In document images, many elements (charts, formulas, and tables) may not be represented using plain text. An increasing number of researchers are now focusing on these element parsing. 
% These elements are often rendered using different formats, such as Markdown, LaTeX, or CSV. 
1) Chart Parsing. Chart types include vertical bars, horizontal bars, lines, scatter plots, and pie charts. Charts serve as visual representations of tables, and organizing text in reading order fails to capture their structure. To preserve their mathematical properties, researchers often convert charts into tables. This process involves breaking down the chart into x/y axes and their corresponding values, which can be represented in Markdown, CSV formats, or even converted into Python code. This approach enables models to better understand the chart's specific meaning.
%%%previous versions
% Chart types include vertical bars, horizontal bars, lines, scatter plots, and pie charts. Charts can be considered as visual representations of tables, and organizing text in reading order does not capture the structure of charts. Therefore, researchers often parse charts into tables to best preserve their mathematical properties. The entire chart can be broken down into x/y axes and their corresponding values. Such data can often be represented in Markdown and CSV formats, and some researchers even convert them into Python code. This approach allows models to gain a deeper understanding of the specific meaning of the entire chart.

2) Table Parsing. Compared to charts, tables have a more standardized structure, where rows and columns form key-value pairs. Common formats for representing tables include LaTeX, Markdown, and HTML. Markdown is often used for simple tables due to its concise text format, while HTML can handle cells that span multiple rows and columns, despite its use of many paired tags like <tr></tr> and <td></td>. Some tables, with complex spanning, custom lines, spacing, or multi-page length, require LaTeX for representation. However, the diversity in LaTeX representations can make these tables challenging for models to fully understand.
%%%previous versions
% Compared to charts, tables have a more standardized structure, where the correspondence between rows and columns represents key-value pairs. Common formats for representing tables include LaTeX, Markdown, and HTML. HTML and Markdown are often used to represent simple tables. Markdown provides a more concise text sequence, whereas, unlike Markdown, HTML can accommodate cells that span multiple rows and columns. However, HTML includes many paired tags, such as '$<tr></tr>$' and '$<td></td>$'. Some tables exceed the representational capabilities of HTML and Markdown, requiring LaTeX for representation. This includes complex row and column spanning, custom table lines and spacing, and multi-page long tables. However, due to the diversity in LaTeX representations, such tables are often challenging for models to truly understand.

3) Formula Parsing. Besides tables and charts, formulas are also commonly used. In the pre-training phase, models learn the LaTeX representation of formula images, enhancing their understanding of formulas. This provides a solid foundation for tasks involving formula computation and reasoning during the instruction alignment.
%%%previous versions
% In addition to tables and charts, formulas are also commonly used data for instruction fine-tuning. During the pre-training phase, models are trained to learn the LaTeX representation of formula images, enhancing the model's understanding of formulas. This lays a solid foundation for tasks involving formula computation and reasoning during the fine-tuning phase.

\subsection{Instruction Alignment}

Upon completing the modality alignment pre-training stage, the MLLM acquires basic visual recognition and dialogue capabilities. However, to achieve human-aligned intelligence, three critical capability gaps must be addressed:(1) Advanced multimodal perception and cross-modal reasoning abilities; (2) Prompt robustness across diverse formulations; (3) Zero-shot generalization for unseen task scenarios. To bridge these gaps, instruction alignment through supervised fine-tuning (SFT) has emerged as an effective paradigm. This phase typically unfreezes all model parameters and employs instructional data with structured templates. 
% Taking visual question answering (VQA) as a representative task, the canonical instruction format is: \texttt{<image><question><answer>}.

To systematically address these challenges, we have categorized the current methods emerging in instruction alignment into three distinct levels:

\noindent \textbf{1) Level 1: Visual-Semantic Anchoring.}  We categorize these instructions into two types: i) Answer within the image; and ii) Answer without the image.
This type of instruction data where answers are located directly within the image, assists MLLMs refine their accuracy in generating responses that are directly linked to specific visual content, reducing reliance on generic or contextually weak answers~\cite{mathew2021docvqa, mathew2022infographicvqa}.
% An example may be: \texttt{<image><question>What is the name of the book?<answer>La La Land.}
Certain tasks require reasoning based on world knowledge and involve complex inference procedures, such as scientific question answering~\cite{masry2022chartqa,chen2021geoqa}. Consequently, these instructions are designed with the common characteristic that the answer is not directly visible in the image. This encourages the model to utilize its linguistic comprehension and external knowledge, enhancing its advanced reasoning and inference capabilities. An example might be: ``Q: How much higher is the red bar compared to the yellow bar in the chart, in terms of percentage? A: 12.1\%.''

\noindent \textbf{2) Level 2: Prompt Diversity Augmentation.} To bolster robustness in handling a broader spectrum of prompts, rather than being limited to specific prompts tailored for particular tasks, researchers often employ data augmentation on the question component of the instruction stream. A popular strategy involves leveraging existing large language models to rephrase the same question in multiple ways. For example, consider the original question: ``What is written on the sign in the image?'' It can be rephrased as: ``Can you read the text displayed on the sign shown in the image?''``Identify the sign in the image.''``Please examine the image and list the words that appear within the sign.''
% \texttt{''What does the text on the sign say?''}
% \texttt{''Look at the sign in the image. What information is provided on its label?''}
% \texttt{''Read the text on the sign.''}
% \texttt{''Observe the sign in the image and describe the text content it contains.''}
By utilizing such varied templates, researchers can train MLLMs to better interpret and respond to a wide range of prompts, thereby enhancing their flexibility and accuracy in real-world applications.

\noindent \textbf{3) Level 3: Zero-shot Generalization.} To enhance the generalization ability to handle unseen tasks, several strategies typically are employed:

Chain of Thought (CoT)~\cite{wei2022chain} reasoning involves breaking down complex problems into a series of intermediate steps or sub-tasks, allowing a model to tackle each part systematically. Some studies have demonstrated improvements by incorporating text-level CoT reasoning~\cite{zhang2024cfret} or box-level visual CoT supervision~\cite{shao2025visual}. To better illustrate the process, consider the prompt: ``What is the average of the last four countries' data?'', the CoT reasoning unfolds as follows: i) Identify the data for the last four countries;
ii) Calculate the sum of these values;
iii) Calculate the average by dividing the sum by the number of countries.
% i) Identify the data for the last four countries: Germany (63), Italy (63), Greece (62), Poland (62);
% ii) Calculate the sum of these values: 63 + 63 + 62 + 62 = 250;
% iii) Calculate the average by dividing the sum by the number of countries: 250 / 4 = 62.5.

Another strategy is Retrieval-Augmented Generation (RAG). RAG~\cite{arslan2024survey} combines the strengths of retrieval-based and generation-based approaches by integrating an information retrieval component with a generative model. This method allows the model to access a vast external knowledge base, retrieving pertinent information to inform and enhance the generation process. 
% For example, consider a scenario where a user asks the question: \texttt{''What are the key achievements of Marie Curie?''}
% i) Retrieval Step: The model first queries a large corpus of scientific articles, biographies, and historical documents to retrieve relevant information about Marie Curie. 
% ii) Generation Step: Using the retrieved information as context, the generative model constructs a detailed response. 

\begin{table*}[!t]
    \centering
    \scalebox{0.9}{
    \input{MLLM_OCR/Table/datawithbench}
    }
    \vspace{-0.5em}
    \caption{Representative datasets and benchmarks for Text-rich Image Understanding. Each dataset is marked for training and testing typically according to its content, functions, and user requirements. 
    % ``Train'' indicates that the dataset is typically used for training. ``Test'' indicates that the dataset is used as an evaluation benchmark. 
    % "Train + Test" indicates that the dataset is divided into both training and benchmark portions.
    }
    \label{tab:datawithbenchmark}
    \vspace{-1.5em}
\end{table*}

\subsection{Preference Alignment}
In the modality and instruction alignment stages, the model predicts the next token based on previous ground-truth tokens during training, and on its own prior outputs during inference. If errors occur in the outputs, this can lead to a distribution shift in inference. The more output the model has, the more serious this phenomenon becomes. In previous natural language processing (NLP) works~\cite{lai2024step,pang2025iterative}, a series of preference alignment techniques~\cite{rafailov2024direct, ouyang2022training,shao2024deepseekmath,wang2024mdpo} have been proposed to optimize the output of the model to make it more consistent with human values and expectations. Benefiting from the success of preference alignment applied to NLP, InternVL2-MPO~\cite{wang2024enhancing} introduces preference alignment to the multimodal field and proposes a Mixed Preference Optimization (MPO) to improve multimodal reasoning. Specifically, they propose a continuation-based Dropout Next Token Prediction (DropoutNTP) pipeline for samples lacking clear ground truth and a correctness-based pipeline for samples with clear ground truth. This strategy improves the performance of the model on OCRBench~\cite{fu2024ocrbench}. Nevertheless, its potential to enhance document multimodal reasoning remains under-explored. 

% To solve this problem, a series of preference alignment techniques have been proposed to optimize the output of the model to make it more consistent with human values and expectations. They include Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training}, Mixed Preference Optimization (MPO)~\cite{wang2024enhancing}, Differential Privacy Optimization (DPO)~\cite{rafailov2024direct}, Group Relative Policy Optimization (GRPO)~\cite{shao2024deepseekmath}, multimodal Direct Preference Optimization (mDPO)~\cite{wang2024mdpo}, \emph{etc.}. 


% Through modality alignment and instruction alignment, MLLM has excellent multimodal understanding, generation, and certain generalization capabilities driven by a large amount of data. However, MLLM still generates inappropriate or unexpected results, often leading to inaccurate, incontextual, or unethical answers.
% \noindent \textbf{RLHF} draws on the idea of reinforcement learning and relies on human feedback to train the model.

% (Reinforcement Learning from Human Feedback) \cite{ouyang2022training} is generally considered a classic work on LLM preference alignment. It draws on the idea of reinforcement learning and relies on human feedback to train the model. The RLHF process consists of two stages: First, the reward model (RM) is trained through human preference data, and then the reward model is used to guide the reinforcement learning optimization of the policy model, in this case, the llMs. RLHF can effectively utilize human preference feedback to better conform the model to human values and expectations. However, it has several notable issues, such as high memory usage, unstable training and complex procedures.

% \noindent \textbf{DPO} (Differential Privacy Optimization) \cite{rafailov2024direct} simplifies the Reinforcement Learning from Human Feedback (RLHF) process, reparameterizes the reward function in the reinforcement learning process and directly learns the policy model from the preference data without an explicit reward model. By incorporating the reward formula into the Bradley-Terry ranking objective, the model is more likely to generate outputs that are acceptable to humans. It simplifies the training process, improves the stability and efficiency of training, and avoids the inconsistency problem between the reward model and the policy model in RLHF. However, DPO cannot fully utilize the reward model and is only applicable to paired preference data, and cannot handle a wider range of feedback types.

% \noindent \textbf{GRPO} (Group Relative Policy Optimization) \cite{shao2024deepseekmath} abandons the traditional Critic model and estimates the advantage function directly through the relative rewards of samples within the group, thereby simplifying the training process and significantly reducing the demand for computing and storage resources. Through relative rewards within the group, GRPO can optimize the strategy more quickly and reduce the variance of strategy updates. Especially when facing complex long-term decision-making problems, it can effectively improve efficiency and ensure a more stable learning process. However, since GRPO needs to sample a set of actions for each state, this may increase the sampling cost in some cases, and GRPO may not be as stable as other methods in some tasks, especially when the reward signal is sparse.

% \noindent \textbf{mDPO} (multimodal Direct Preference Optimization) \cite{wang2024mdpo} is a preference optimization method for multimodal large language models, which aims to address the shortcomings of DPO for image modalities in multimodal scenarios. mDPO introduces new image preference pairs and an image-based reward anchoring mechanism, which effectively solves the unconditional preference problem in multimodal preference optimization, that is, the problem in which the model ignores the image conditions during the optimization process. By introducing image preference pairs, mDPO can better utilize visual information, improve the model's ability to understand images, significantly reduce the hallucination output of MLLM, and improve model performance. However, due to the introduction of image preference comparison, mDPO will bring additional memory and computational costs during the optimization process, which is usually more than twice that of DPO under the same circumstances.


==> MLLM_OCR/sec/4_dataset.tex <==
\section{Datasets and Benchmarks}
\label{sec:datasets}

% \textcolor{red}{The evolution of text-rich image understanding tasks is profoundly intertwined with the proliferation of publicly available datasets and benchmarks, where dataset construction manifests a dual trajectory of scenario specialization and task sophistication. Contemporary datasets predominantly center on six pivotal domains: document, chart, natural scene, table, mathematical reasoning, and graphical user interface (GUI) interaction, addressing multi-tiered demands spanning from single-page document parsing to cross-page contextual reasoning, and from elementary information retrieval to advanced logical computations.}

The rapid advancements in TIU tasks have been fundamentally driven by the proliferation of specialized datasets and standardized benchmarks. As illustrated in Table \ref{tab:datawithbenchmark}, we systematically categorize TIU-related datasets into two types: \textit{domain-specific} (Document, Chart, Scene, Table, and GUI) and \textit{comprehensive} scenarios. 
%This taxonomy not only reflects the evolving landscape of TIU research but also highlights the community's focused efforts on addressing domain-specific challenges through targeted dataset creation.

% \textcolor{red}{Key considerations in dataset design include image scale, diversity of question-answer pairs, annotation quality, and applicability to real-world scenarios. These factors are critical for creating datasets that are comprehensive and accurately represent the challenges faced in Text-Image Understanding (TIU) tasks.} 

Specifically, some datasets are derived by converting training data from traditional tasks~\cite{guan2022industrial,guan2023self} into Visual Question Answering (VQA) formats, such as text detection, text spotting, table recognition, and \emph{etc.}. These datasets are typically utilized for modality alignment in the first stage of training, enabling models to bridge the gap between textual and visual information effectively. Other datasets are specifically designed in VQA formats for certain scenarios, such as DocVQA~\cite{mathew2021docvqa}, InfoVQA~\cite{mathew2022infographicvqa}, ChartQA~\cite{masry2022chartqa}, and TextVQA~\cite{singh2019towards}. These datasets have played a pivotal role in advancing the field of TIU by providing structured and domain-specific challenges. Their introduction has significantly accelerated progress in tasks like document understanding, chart interpretation, and natural scene text comprehension. Consequently, published papers frequently report these metrics, as they not only contribute to instruction alignment in the second stage of training but also serve as essential benchmarks for evaluating model performance.

In addition to training datasets, there is a distinct category of datasets that are exclusively designed for evaluating specific capabilities of MLLMs. Examples include TableVQA-Bench~\cite{Kim2024ARXIV_TableVQA_Bench_A}, ChartBench~\cite{Xu2024ARXIV_ChartBench_A_Benchmark}, and MMLongBench-Doc~\cite{Ma2024NEURIPS_MMLongBench_Doc_Benchmarking}. These datasets are tailored to assess advanced functionalities such as long-context understanding, cross-modal reasoning, and domain-specific comprehension. By providing targeted evaluation frameworks, they enable researchers to identify strengths and weaknesses in MLLMs, driving further innovation and refinement in the field.


% \begin{table*}[t]
%     \centering
%     \scalebox{0.95}{
%     \input{Table/dataset}
%     }
%     \caption{Representative datasets designed for rich text image understanding in different scenes}
%     \label{tab:my_label}
% \end{table*}

% % benchmark
% \begin{table*}[t]
%     \centering
%     \scalebox{0.95}{
%     \input{MLLM_OCR/Table/benchmark}
%     }
%     \caption{Publicly available evaluation benchmarks designed for rich text image understanding in different scenes}
%     \label{tab:benchmark}
% \end{table*}

==> MLLM_OCR/sec/5_summary.tex <==
%展望未来及 MLLM for VDU 的应用场景
\section{Challenges and Trends}
\label{sec:summary}

%According to the evolutionary trends of model architectures shown in Table \ref{tab:mllm_summary}, it can be observed that the model structures are beginning to evolve in two directions: 1. The number of model parameters is decreasing. For instance, Mini-monkey, with 2B parameters, has achieved results comparable to those of 7B models on multiple TIU tasks. 2. Models are capable of processing longer inputs. For example, DocOwl2.0, by compressing visual tokens, can handle more input images while maintaining the same performance metrics. In terms of training strategies, in addition to MA and IA, PA is also being introduced to enhance the model's question-answering capabilities and overall performance. Moreover, it is conceivable that with the ongoing popularity of reinforcement learning sparked by DeepSeek R1, training strategies using GRPO will also emerge during the PA phase in the MLLM field.

As shown in Table \ref{tab:mllm_summary}, we calculated the average scores from four popular and widely used evaluation datasets, which can basically reflect the performance of MLLMs on TIU tasks. The top five models are Qwen2-VL-72B (88.70), InternVL2.5-78B (87.73), InternVL2.5-38B (87.45), InternVL2.5-26B (85.85), and DeepSeek-VL2-27B (85.40). This indicates that the most state-of-the-art (SOTA) MLLMs currently employ OCR-free encoders, which avoids redundant tokens and complex model architectures. Despite the promising and significant progress made by current MLLMs, the field still faces considerable challenges that require further research and innovation:

% the latest MLLM model architectures predominantly adopt an OCR-free encoder and  Qwen LLM, achieving significant progress on mainstream benchmarks. For instance, the metric on DocVQA has reached a peak of 96.5\%. However, the field still faces significant challenges that demand further research and innovation:

\noindent \textbf{Computational Efficiency and Model Compression}. The computational demands of current MLLMs remain a critical bottleneck, primarily due to two factors: (1) the necessity of processing high-resolution document images, which imposes substantial computational resource requirements, and (2) the prevalent use of 7-billion-parameter architectures, while delivering state-of-the-art performance, incur high deployment costs and latency. These challenges underscore the importance of developing more efficient MLLM architectures that balance performance with reduced computational overhead. Encouragingly, recent advancements, as illustrated in Table~\ref{tab:mllm_summary}, demonstrate promising trends toward model miniaturization. For instance, Mini-monkey~\cite{Huang2024ARXIV_Mini_Monkey_Alleviating} achieves performance comparable to 7B-parameter models on multiple TIU tasks while utilizing only 2B parameters, highlighting the potential for lightweight yet powerful architectures.

\noindent \textbf{Optimization of Visual Feature Representation}. A persistent challenge in MLLMs is the disproportionate length of image tokens compared to text tokens, which significantly increases computational complexity and degrades inference efficiency. Addressing this issue requires innovative approaches to compress image tokens without sacrificing model performance. Promising directions include the development of efficient visual encoders, adaptive token compression mechanisms, and advanced techniques for cross-modal feature fusion. Crucially, these methods must preserve the semantic richness of document content during compression. As shown in Table~\ref{tab:mllm_summary}, recent architectural innovations, such as mPLUG-DocOwl2‘s ~\cite{Hu2024ARXIV_mPLUG_DocOwl2_High} visual token compression, have made strides in this direction by enabling the processing of larger input images while maintaining benchmark performance.

\noindent \textbf{Long Document Understanding Capability}. While MLLMs excel at single-page document understanding, their performance on multi-page or long-document tasks remains suboptimal. Key challenges include modeling long-range dependencies, maintaining contextual coherence across pages, and efficiently processing extended sequences. The emergence of specialized benchmarks for long-document understanding~\cite{Ma2024NEURIPS_MMLongBench_Doc_Benchmarking}, as highlighted in Table~\ref{tab:datawithbenchmark}, is expected to drive significant progress in this field by providing standardized evaluation frameworks and fostering targeted research efforts.

\noindent \textbf{Multilingual Document Understanding}. Current MLLMs are predominantly optimized for English and a limited set of high-resource languages, resulting in inadequate performance in multilingual and low-resource language scenarios. Addressing this limitation requires the development of comprehensive multilingual datasets that encompass diverse linguistic and cultural contexts. Recent initiatives, such as MT-VQA~\cite{tang2024mtvqa} and CC-OCR~\cite{yang2024cc} (referenced in Table~\ref{tab:datawithbenchmark}), represent important steps forward by introducing TIU tasks specifically designed to evaluate multilingual capabilities. These efforts, coupled with advances in cross-lingual transfer learning, are expected to significantly enhance the inclusivity and applicability of MLLMs in global contexts.

%\noindent \textbf{Evaluation Standards and New Benchmarks}. The current evaluation standards for TIU tasks are predominantly based on limited benchmark datasets, which may not fully capture the model's performance in real-world scenarios, especially the reasoning ablity. Furthermore, the existing evaluation metrics are often overly simplistic, lacking the ability to comprehensively assess the model's multidimensional capabilities. To address these limitations, it is crucial to develop more comprehensive evaluation benchmarks that encompass a diverse range of document types, languages, and domains.

==> MLLM_OCR/sec/6_limitation.tex <==
\section{Limitations}

This paper provides a systematic review of multimodal large language models (MLLMs) in the field of Text-rich Image Understanding (TIU). While the research team has conducted comprehensive retrieval and integration of core literature prior to the submission deadline, certain minor studies may still remain uncovered. It should be particularly noted that due to publisher formatting requirements, the exposition of existing technical approaches and benchmark datasets in this work maintains essential conciseness. For complete algorithmic implementation details and experimental parameter configurations, researchers are strongly recommended to consult the original publications.

%按场景介绍TIU 领域常用的 benchmark， eval metrics，
%分析当前 benchmark 存在的问题后，提出新的 benchmark，并提供当前已知可测试的 MLLM 模型在这个 benchmark 的结果





% \subsection{Evaluation metrics}
% Evaluation metrics play a critical role in assessing the performance of MLLM across various tasks and benchmarks. They include Precision, Recall, F1 Score, Accuracy, MAP, and ANLS. More details will be introduced in Supplemental Martial.
% Specifically, we introduce the important ANLS metric in detail:

% The key evaluation metrics are as follows:

% \textcolor{red}{\subsubsection{Precision, Recall, F1 Score, and Accuracy}}

% Precision, Recall, F1 Score, and Accuracy are pivotal in assessing model performance across diverse tasks.

% \noindent \textbf{Precision} measures the model's ability to correctly identify positive instances within multi-modal data. This metric is calculated as follows:
% \begin{gather}
%     \mathrm{Precision}=\frac{\text{TP}}{\text{TP}+\text{FP}}
% \end{gather}

% \noindent \textbf{Recall} evaluates the model's capability to identify all relevant positive instances in multi-modal tasks. This metric is calculated as follows:
% \begin{gather}
%     \mathrm{Recall}=\frac{\text{TP}}{\text{TP}+\text{FN}}
% \end{gather}

% \noindent \textbf{F1 Score}, as the harmonic mean of precision and recall, is particularly valuable in scenarios where a balance between these two metrics is desired. This metric is calculated as follows:
% \begin{gather}
%     \mathrm{F1~Score}=\frac{2\times\mathrm{Precision}\times\mathrm{Recall}}{\mathrm{Precision}+\mathrm{Recall}}
% \end{gather}

% \noindent \textbf{Accuracy} represents the proportion of correctly predicted observations and is the most straightforward performance metric. This metric is calculated as follows:
% \begin{gather}
%     \mathrm{Accuracy}=\frac{\text{TP}+\text{TN}}{\text{Total Samples}}
% \end{gather}
% Where, TP (TP) are the correctly predicted positive samples. FP (FP) are the incorrectly predicted positive samples. FN (FN) are the incorrectly predicted negative samples. TN (TN) are the correctly predicted negative samples. Total Samples is the total number of samples
% in the dataset.

% \subsubsection{Mean Average Precision (MAP)}
% MAP is employed to evaluate the precision of retrieval tasks involving multi-modal data, such as retrieving the most relevant images from a database based on a given text description. MAP is employed to evaluate the precision of retrieval tasks involving multi-modal data, such as retrieving the most relevant images from a database based on a given text description.  MAP effectively measures the model's average performance across multiple queries, ensuring the model excels not only in isolated instances but consistently. MAP effectively measures the model's average performance across multiple queries, ensuring the model excels not only in isolated instances but consistently. The formula for calculating MAP is as follows:
% \begin{gather}
% \mathrm{MAP}=\frac{1}{Q}\sum_{q=1}^Q\mathrm{AP}(q)
% \end{gather}
% Where, $Q$ is the total number of queries. $\mathrm{AP}(q)$ is the Average Precision for query $q$, calculated as the average precision of relevant documents at each position in the ranked list:
% \begin{gather}
% \mathrm{AP}(q)=\frac{1}{N_q}\sum_{k=1}^{N_q}\mathrm{Precision}(k)\times\mathrm{Relevance}(k)
% \end{gather}
% Where, $N_q$ is the total number of retrieved documents for query $q$. $\mathrm{Precision}(k)$ is the precision at position $k$ in the ranked list. $\mathrm{Relevance}(k)$ is an indicator function that
% takes the value 1 if the document at position
% $k$ is relevant to query $q$, and 0 otherwise.

% \textcolor{red}{\subsubsection{Average Normalized Levenshtein Similarity (ANLS)}}
% ANLS~\cite{biten2019scene} captures the OCR mistakes applying a slight penalization in case of correct intended responses, but badly recognized. It also makes use of a threshold of value 0.5 that dictates whether the output of the metric will be the ANLS if its value is equal to or bigger than 0.5 or 0 otherwise. The key point of this threshold is to determine if the answer has been correctly selected but not properly recognized, or on the contrary, the output is a wrong text selected from the options and given as an answer.

% More formally, the ANLS between the net output and the ground truth answers is given by the following equation. Where $N$ is the total number of questions, $M$ total number of GT answers per question, $a_{ij}$ the ground truth answers where $i = {0, ..., N}$, and $j = {0, ..., M}$, and $o_{qi}$ be the network’s answer for the ith question $q_i$:
% \begin{gather}
% \mathrm{ANLS}=\frac{1}{N} \sum_{i=0}^N\left(\max _j s\left(a_{i j}, o_{q i}\right)\right)
% \end{gather}
% Where, $s\left(a_{i j}, o_{q i}\right)$ is defined as follows:
% \begin{gather}
% s\left(a_{i j}, o_{q i}\right)= \begin{cases}1-\mathrm{NL}\left(a_{i j}, o_{q i}\right), & \text { if } \mathrm{NL}\left(a_{i j}, o_{q i}\right)< \tau\\ 0, & \text { if } \mathrm{NL}\left(a_{i j}, o_{q i}\right) \geq\tau \end{cases}
% \end{gather}



==> Table/benchmark.tex <==
\scriptsize
    \begin{tabular}{cccccccc}
    \toprule
    Types & Benchmark & Language &\#Scenario & \#Task & \#Num & \#Instruction &Open-source  \\
    \midrule
    \multirow{3}{*}{Document} 
    & OCREval~\cite{lv2023kosmos} & English & Multi-domain & 1 & 2,297 & - & \ding{51}\\
    & MMLongBench-Doc~\cite{Ma2024NEURIPS_MMLongBench_Doc_Benchmarking} & English & Multi-domain Long Documents & 3 & 135 & 1k & \ding{51}\\
    & Do-GOOD~\cite{He2023ARXIV_Do_GOOD_Towards} & English & Industry document  & 3 & 410k & 50k & \ding{51}\\
    \midrule 
    \multirow{4}{*}{Chart }& ChartY~\cite{chen2024onechart} & English,Chinese & Charts and Plots  & 1 & 6k & 6k & \ding{51}\\
    & ChartX~\cite{xia2024chartx} & English & Charts and Plots & 7 & 6k & 6k & \ding{51}\\
    & MMC~\cite{Liu2024NAACL_MMC_Advancing_Multimodal} & English & Plots (Real world data source) & 9 & 1.7k& 2.9k & \ding{55}\\
    & ChartBench~\cite{Xu2024ARXIV_ChartBench_A_Benchmark} & English & Plots (Real world data source) & 2 & 68k& 549k & \ding{55}\\
    \midrule  
    \multirow{3}{*}{Table} & TableVQA-Bench~\cite{Kim2024ARXIV_TableVQA_Bench_A} & English & Scientific and Financial Reports & 3 & 0.9k & 1.5k & \ding{51}\\
    & MMTab-eval~\cite{zheng2024multimodal} & English & Scientific and Financial Reports & 9 & 23k & 49k & \ding{51}\\
    & ComTQA~\cite{Zhao2024NEURIPS_TabPedia_Towards_Comprehensive} & English & Scientific and Financial Reports & 4 & 1.6k & 9k & \ding{51}\\
    \midrule 
    \multirow{1}{*}{GUI} 
    & Screen2Words~\cite{wang2021screen2words} & English & Android app screenshot & 1 & 22k & 112k & \ding{51}\\
    \midrule 
    \multirow{8}{*}{Synthesis} & OCRbench~\cite{liu2024ocrbench} & English & Multi-domain & 5 & 0.9k & 1k & \ding{51}\\
    & Seed-bench-2-plus~\cite{li2024seed} & English & Multi-domain & 1 & 0.6k & 2.3k & \ding{51}\\
    & CONTEXTUAL~\cite{wadhawan2024contextual} & English & Multi-domain & 1 & 0.5k & 0.5k & \ding{51}\\
    & OCRBench v2~\cite{fu2024ocrbench} & English & Multi-domain & 23 & 9.5k & 10k & \ding{51}\\
    & FOX~\cite{liu2024focus} & English,Chinese & Academic Document Corpus & 9 & 0.7k & 2.2k & \ding{51}\\
    & DocLocal4K~\cite{hu-etal-2024-mplug} & English & Multi-domain & 2 & 4.2k & 4.2k & \ding{51}\\
    & CC-OCR~\cite{yang2024cc} & Multilingual & Multi-domain & 3 & 7k & - & \ding{51}\\
    & MMDocBench~\cite{Zhu2024ARXIV_MMDocBench_Benchmarking_Large} & English & Multi-domain & 15 & 2.4k & 4.3k & \ding{51}\\
    
    \bottomrule
    \end{tabular}

==> Table/dataset.tex <==
\scriptsize
    \begin{tabular}{llccccc}
    \toprule
    Types & Dataset & Language & Scene Sources & \#Images & \#Q\&A pairs & Answer in Picture \\
    \midrule
    \multirow{4}{*}{Document} & DocVQA~\cite{mathew2021docvqa} & English & Industry document & 12,767&  50,000 & Yes\\
    & Docmatix~\cite{laurenccon2024building} & English & Industry document & 2.4M & 9.5M & Yes\\
    & InfoVQA~\cite{mathew2022infographicvqa} & English & Infographics & 5,485 & 30,035 & Yes\\
    & MP-DocVQA~\cite{tito2023hierarchical} & English & Industry documents & 47,952 & 46,176 & Yes\\
    &DocGenome~\cite{xia2024docgenome} & English & Scientific document & 6.8M & 3,000 & Yes\\
    &IIT-CDIP~\cite{xu2020layoutlm} & English & Multi-domain & 11M & - & -\\
    &synthdog~\cite{kim2022ocr}& English & Multi-domain & 2M & - & -\\
    &CCPdf~\cite{turski2023ccpdf}& Multiple languages & Multi-domain & 1.1M & - & - \\
    \midrule 
    \multirow{4}{*}{Chart }& ChartQA~\cite{masry2022chartqa} & English & Charts and Plots  & 20,882 & 32,719 & Yes\\
    & PlotQA~\cite{methani2020plotqa} & English & Plots (Real world data source) & 224,377 & 28.9M & Yes\\
    & FigureQA~\cite{kahou2017figureqa} & English & Science style image & over 100,000 & over 1.3M& Yes\\
    & DVQA~\cite{kafle2018dvqa} & English & Data Visualizations & 300,000 & 3,487,194 & Yes\\
    \midrule 
    \multirow{4}{*}{Scene} & TextCaps~\cite{sidorov2020textcaps} & English & Scene Text (Open Images) & 28,408 & 142,040 & Yes\\
    & TextVQA~\cite{singh2019towards} & English & Scene Text (Open Images) & 28,408 & 45,336 & Yes\\
    & ST-VQA~\cite{biten2019scene} & English & Scene Text & 23,038 & 31,791 & Yes\\
    & MT-VQA~\cite{wen2024mt} & Multiple languages & 20 fine-grained scenes & 8,794 & 28,607 & Yes\\
    \midrule 
    \multirow{1}{*}{Table} & TableQA~\cite{sun2020tableqa} & English & Financial reports & 6,000 & 64,891 & Yes\\
    &WikiTableQuestions~\cite{pasupat2015compositional}& English & Multi-domain & 2,108 & 22,033 & Yes\\
    &DeepForm~\cite{svetlichnaya2020deepform}& English & Political campaign finance receipts & 20,000 & - & - \\
    \midrule 
    \multirow{2}{*}{Math} & GeoQA~\cite{chen2021geoqa} & Chinese & Mathematics test questions & 5,010 & 5,010 & No\\
    & GeoQA+~\cite{cao2022augmented} & Chinese & Online education website & 12,054 & 12,054 & No\\
    % \midrule 
    % \multirow{1}{*}{Code}&&&&&&\\
    % &&&&&&\\
    \midrule 
    \multirow{2}{*}{GUI} & ScreenQA~\cite{hsiao2022screenqa} & English & Mobile app screenshots & 35,352 & 85,984 & Yes\\
    & Screen2Words~\cite{wang2021screen2words} & English & Android app screenshot & 22,417 & 112,085 & No\\
    \bottomrule
    \end{tabular}



==> Table/datawithbench.tex <==
\scriptsize
    \begin{tabular}{l|>{\centering\arraybackslash}m{4.2cm}|>{\centering\arraybackslash}m{1.2cm}|>{\centering\arraybackslash}m{3.5cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1.5cm}}
    \toprule
    Domain & Dataset & Language & Scene Sources & \#Images & \#Q\&A pairs & Train/Test \\
    \midrule
    \multirow{25}{*}{Document} & DocVQA~\cite{mathew2021docvqa} & English & Industry document & 12,767&  50,000 & Train + Test \\
    & Docmatix~\cite{laurenccon2024building} & English & Industry document & 2.4M & 9.5M & Train \\
    & InfoVQA~\cite{mathew2022infographicvqa} & English & Infographics & 5,485 & 30,035 & Train + Test \\
    & MP-DocVQA~\cite{tito2023hierarchical} & English & Industry documents & 47,952 & 46,176 & Train + Test \\
    &DocGenome~\cite{xia2024docgenome} & English & Scientific document & 6.8M & 3,000 & Train \\
    &IIT-CDIP~\cite{xu2020layoutlm} & English & Multi-domain & 11M & - & Train \\
    &synthdog~\cite{kim2022ocr}& English & Multi-domain & 2M & - & Train \\
    &CCPdf~\cite{turski2023ccpdf}& Multilingual & Multi-domain & 1.1M & - & Train \\
    &RVL-CDIP~\cite{harley2015evaluation} & English & Industry document & 159,418 & - & Train \\
    &VisualMRC~\cite{tanaka2021visualmrc} & English & Webpage Document & 10,197 & 30,562 & Train + Test \\
    &KLC~\cite{stanislawek2021kleister} & English & Industry document & 2463 & 22,224 & Train + Test \\
    & OCREval~\cite{lv2023kosmos} & English & Multi-domain & 2,297 & - & Test \\
    & MMLongBench-Doc~\cite{Ma2024NEURIPS_MMLongBench_Doc_Benchmarking} & English & Multi-domain Long Documents & 135 & 1k & Test \\
    & Do-GOOD~\cite{He2023ARXIV_Do_GOOD_Towards} & English & Industry document & 410k & 50k & Test\\
    & OCR-VQA~\cite{mishra2019ocr} & English & Book covers & 207,572 & >1M & Train + Test\\
    & SlideVQA~\cite{tanaka2023slidevqa} & English & Slide decks & 52,480 & 14,484 & Train + Test\\
    & PDF-VQA~\cite{10.1007/978-3-031-43427-3_35} & English & Scientific document  & 13,484 & 140,610 & Train + Test\\
    & BenthamQA~\cite{mathew2021asking} & English & Handwritten document  & 338 & 200 & Train + Test\\
    & FinanceQA~\cite{Sujet-Finance-QA-Vision-100k} & English & Financial reports & 9,801 & 100k & - \\
    & Ureader~\cite{ye-etal-2023-ureader} & English & Multi-domain & 24.5k & 24.5k & Train \\
    & ColPali~\cite{faysse2024colpali} & English & Multi-domain & 118,695 & 118,695 & Train + Test \\
    & FUNSD~\cite{jaume2019funsd} & English & Scanned forms & 199 & 5312 & Train + Test \\
    & SROIE~\cite{huang2019icdar2019sroie} & English & Multi-domain & 973 & 52,316 & Train + Test \\
    & POIE~\cite{kuang2023visual} & English & Multi-domain & 3,000 & 111,155 & Train + Test \\
    & IAM~\cite{marti2002iam} & English & Lancaster-Oslo/Bergen & 1066 & - & Train \\
    \midrule 
    \multirow{12}{*}{Chart}& ChartQA~\cite{masry2022chartqa} & English & Charts and Plots  & 20,882 & 32,719 & Train + Test\\
    & PlotQA~\cite{methani2020plotqa} & English & Plots (Real world data source) & 224,377 & 28.9M & Train \\
    & FigureQA~\cite{kahou2017figureqa} & English & Science style image & >100,000 & >1.3M& Train \\
    & DVQA~\cite{kafle2018dvqa} & English & Data Visualizations & 300,000 & 3,487,194 & Train \\
    & Unichart~\cite{masry2023unichart} & English & Multi-domain & 290,736 & 300,000 & Train \\
    & LRV-Instruction~\cite{liu2023mitigating} & English & Multi-domain & 400k & 400k & Train + Test  \\
    & VisText~\cite{tang-etal-2023-vistext} & English & Financial reports & 12,441  & 12,441 & Train + Test \\
    & Chart2Text~\cite{obeid-hoque-2020-chart} & English & Financial reports & 8,305 & 8,305 & Train + Test \\
    & ArxivQA~\cite{li-etal-2024-multimodal-arxiv} & English & Scientific Chart & 35,000 & 100,000 & Train + Test \\

    & ChartY~\cite{chen2024onechart} & Multilingual & Charts and Plots & 6k & 6k & Test \\
    & ChartX~\cite{xia2024chartx} & English & Charts and Plots & 6k & 6k & Test\\
    & MMC~\cite{Liu2024NAACL_MMC_Advancing_Multimodal} & English & Plots (Real world data source) & 1.7k& 2.9k & Test\\
    & ChartBench~\cite{Xu2024ARXIV_ChartBench_A_Benchmark} & English & Plots (Real world data source) & 68k& 549k & Test \\
    
    \midrule 
    \multirow{13}{*}{Scene} & TextCaps~\cite{sidorov2020textcaps} & English & Scene Text & 28,408 & 142,040 & Train + Test \\
    & TextVQA~\cite{singh2019towards} & English & Scene Text & 28,408 & 45,336 & Train + Test \\
    & ST-VQA~\cite{biten2019scene} & English & Scene Text & 23,038 & 31,791 & Train + Test \\
    & MT-VQA~\cite{wen2024mt} & Multilingual & 20 fine-grained scenes & 8,794 & 28,607 & Train + Test \\
    & OCRVQA~\cite{mishra2019ocr} & English & Scene Text & 207,572 & 1M & Train \\
    & ICDAR13~\cite{karatzas2013icdar} & English & Scene Text & 229 & - & Train \\
    & ICDAR15~\cite{karatzas2015icdar} & English & Scene Text & 1000 & - & Train \\
    & TotalText~\cite{ch2017totaltext} & English & Scene Text & 1000 & - & Train \\
    & CTW1500~\cite{yuliang2017detecting} & English & Scene Text & 1255 & - & Train \\
    & LSVT~\cite{sun2019icdar} & Chinese & Scene Text & 30,000 & - & Train \\
    & RCTW~\cite{shi2017icdar2017} & Chinese & Scene Text & 8,034 & - & Train \\
    &LAION-OCR~\cite{schuhmann2022laion} & English & Scene Text & - & - & Train \\
    &Wukong-OCR~\cite{gu2022wukong} &Chinese & Scene Text & - & - & Train\\
    \midrule 
    \multirow{13}{*}{Table} & TableQA~\cite{sun2020tableqa} & English & Financial reports & 6,000 & 64,891 & Train \\
    &WikiTableQuestions~\cite{pasupat2015compositional}& English & Multi-domain & 2,108 & 22,033 & Train + Test\\
    &DeepForm~\cite{svetlichnaya2020deepform}& English & Political campaign finance receipts & 1100 & 5500 & Train + Test \\
    &TabFact~\cite{chen2019tabfact} & English & Wikipedia tables & 14,922 & 117,273 & Train + Test \\
    &TabMWP~\cite{lu2022dynamic} & English & Educational documents & 38,431 & 38,431 & Train \\
    &TURL~\cite{deng2022turl} & English & Wikipedia & 200,000 & - & Train \\
    &PubTabNet~\cite{zhong2020image} & English & Scientific articles & 200,000 & - & Train \\
    & TableVQA-Bench~\cite{Kim2024ARXIV_TableVQA_Bench_A} & English & Scientific and Financial Reports & 0.9k & 1.5k & Test \\
    & MMTab-eval~\cite{zheng2024multimodal} & English & Scientific and Financial Reports & 23k & 49k & Test \\
    & ComTQA~\cite{Zhao2024NEURIPS_TabPedia_Towards_Comprehensive} & English & Scientific and Financial Reports & 1.6k & 9k & Test \\
    & TAT-DQA~\cite{zhu2022towards} & English & Financial reports & 3,067 & 16,558 & Train + Test \\
    & VQAonBD~\cite{raja2023icdar} & English & Financial reports & 48,895 & 1,531,455 & Train + Test \\
    & MultiHiertt~\cite{zhao-etal-2022-multihiertt} & English & Financial reports & 89,646 & 10,440 & Train + Test \\

    % \midrule 
    % \multirow{2}{*}{Math} & GeoQA~\cite{chen2021geoqa} & Chinese & Mathematics test questions & 5,010 & 5,010 & No\\
    % & GeoQA+~\cite{cao2022augmented} & Chinese & Online education website & 12,054 & 12,054 & No\\
    % \midrule 
    % \multirow{1}{*}{Code}&&&&&&\\
    % &&&&&&\\
    \midrule 
    \multirow{2}{*}{GUI} & ScreenQA~\cite{hsiao2022screenqa} & English & Mobile app screenshots & 35,352 & 85,984 & Train + Test\\
    & Screen2Words~\cite{wang2021screen2words} & English & Android app screenshot & 22,417 & 112,085 & Train + Test \\
    \midrule 
    \multirow{8}{*}{Comprehensive} & OCRbench~\cite{liu2024ocrbench} & English & Multi-domain & 0.9k & 1k & Test\\
    & Seed-bench-2-plus~\cite{li2024seed} & English & Multi-domain & 0.6k & 2.3k & Test \\
    & CONTEXTUAL~\cite{wadhawan2024contextual} & English & Multi-domain & 0.5k & 0.5k & Test \\
    & OCRBench v2~\cite{fu2024ocrbench} & English & Multi-domain & 9.5k & 10k & Test\\
    & FOX~\cite{liu2024focus} & Multilingual & Scientific document  & 0.7k & 2.2k & Test\\
    & DocLocal4K~\cite{hu-etal-2024-mplug} & English & Multi-domain & 4.2k & 4.2k & Test\\
    & CC-OCR~\cite{yang2024cc} & Multilingual & Multi-domain & 7k & - & Test\\
    & MMDocBench~\cite{Zhu2024ARXIV_MMDocBench_Benchmarking_Large} & English & Multi-domain & 2.4k & 4.3k & Test\\
    \bottomrule
    \end{tabular}


